On-line Chain Partitions of Up-growing Semi-orders

On-line chain partition is a two-player game between Spoiler and Algorithm. Spoiler presents a partially ordered set, point by point. Algorithm assigns incoming points (immediately and irrevocably) to the chains which constitute a chain partition of the order. The value of the game for orders of width $w$ is a minimum number $\fVal(w)$ such that Algorithm has a strategy using at most $\fVal(w)$ chains on orders of width at most $w$. We analyze the chain partition game for up-growing semi-orders. Surprisingly, the golden ratio comes into play and the value of the game is $\lfloor\frac{1+\sqrt{5}}{2}\; w \rfloor$.

==> pictures/fig-B_0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Mar 11 23:23:32 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="63.12" y-min="0" y-max="23.38" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 points= "(30,5);(30,5);(30,12);(30,12);(30,12);(0,5);
%	(0,5);(0,5);(30,5)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#dcdcdc"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(30,12.5);(30,12.5)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 />
%<parallelogram p3= "(30,0)"
%	 p2= "(30,5)"
%	 p1= "(-0,5)"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(21.25,13.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<multicurve fill-style= "solid"
%	 points= "(63.12,10);(63.12,10);(63.12,5);(63.12,5);(63.12,5);(0,5);
%	(0,5);(0,5);(35,10);(35,10);(35,10);(63.12,10)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#c0c0c0"
%	 />
%<circle p3= "(30.62,13.12)"
%	 p2= "(29.38,13.12)"
%	 p1= "(29.38,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,15)"
%	 fill-style= "none"
%	 stroke-color= "#808080"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$p_n$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.25,11.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,2.5)"
%	 fill-style= "none"
%	 stroke-color= "#808080"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$p_n\oDownset$
%</text>
%<parallelogram p3= "(63.12,0)"
%	 p2= "(63.12,5)"
%	 p1= "(30,5)"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#f0f0f0"
%	 />
%<parallelogram p3= "(63.12,10)"
%	 p2= "(63.12,15)"
%	 p1= "(35,15)"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(59.37,2.5);(59.37,2.5);(59.37,22.5);(59.37,22.5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.12,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "center-h"
%	 >
%$B_0$
%</text>
%<circle p3= "(60,13.12)"
%	 p2= "(58.74,13.12)"
%	 p1= "(58.74,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(60,3.12)"
%	 p2= "(58.74,3.12)"
%	 p1= "(58.74,1.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(60,23.12)"
%	 p2= "(58.74,23.12)"
%	 p1= "(58.74,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(63.12,23.38)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](30,5)
(30,12)
(0,5)(30,5)
\psline[linewidth=0.05,linecolor=gray](30,5)(30,12.5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](-0,5)(30,5)(30,0)(0,0)
\rput(21.25,13.75){}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=lightgray,fillstyle=solid](63.12,10)
(63.12,5)
(0,5)
(35,10)(63.12,10)
\rput{0}(30,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(26.25,15){$p_n$}
\rput(31.25,11.25){}
\rput(15,2.5){$p_n\oDownset$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](30,5)(63.12,5)(63.12,0)(30,0)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](35,15)(63.12,15)(63.12,10)(35,10)
\psline[linewidth=0.15](59.37,2.5)(59.37,22.5)
\rput(48.12,12.5){$B_0$}
\rput{0}(59.37,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(59.37,2.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(59.37,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\end{pspicture}


==> pictures/fig-claim-f.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Mar 11 23:19:31 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="52.5" y-min="0" y-max="23.38" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 points= "(22.5,5);(22.5,5);(22.5,12.5);(22.5,12.5);(22.5,12.5);(0,5);
%	(0,5);(0,5);(22.5,5)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#dcdcdc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(37.5,5);(37.5,5);(37.5,12.5);(37.5,12.5);(37.5,12.5);(0,5);
%	(0,5);(0,5);(37.5,5)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#c0c0c0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,22.5);(22.5,22.5);(22.5,12.5);(22.5,12.5)"
%	 stroke-width= "0.05"
%	 />
%<parallelogram p3= "(52.5,0)"
%	 p2= "(52.5,5)"
%	 p1= "(37.5,5)"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#f0f0f0"
%	 />
%<parallelogram p3= "(22.5,0)"
%	 p2= "(22.5,5)"
%	 p1= "(-0,5)"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(21.25,13.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<circle p3= "(23.12,13.12)"
%	 p2= "(21.88,13.12)"
%	 p1= "(21.88,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(23.12,23.12)"
%	 p2= "(21.88,23.12)"
%	 p1= "(21.88,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<parallelogram p3= "(37.5,0)"
%	 p2= "(37.5,5)"
%	 p1= "(22.5,5)"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(37.5,12.5);(37.5,12.5)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 />
%<circle p3= "(38.12,13.12)"
%	 p2= "(36.87,13.12)"
%	 p1= "(36.87,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,12.5)"
%	 fill-style= "none"
%	 stroke-color= "#808080"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$b$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,12.5)"
%	 fill-style= "none"
%	 stroke-color= "#808080"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$p_n$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(12.5,2.5)"
%	 fill-style= "none"
%	 stroke-color= "#808080"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$b\oDownset$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(52.5,23.38)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](22.5,5)
(22.5,12.5)
(0,5)(22.5,5)
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=lightgray,fillstyle=solid](37.5,5)
(37.5,12.5)
(0,5)(37.5,5)
\psline[linewidth=0.05](22.5,22.5)(22.5,12.5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](37.5,5)(52.5,5)(52.5,0)(37.5,0)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](-0,5)(22.5,5)(22.5,0)(0,0)
\rput(21.25,13.75){}
\rput{0}(22.5,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(22.5,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](22.5,5)(37.5,5)(37.5,0)(22.5,0)
\psline[linewidth=0.05,linecolor=gray](0,5)(37.5,12.5)
\rput{0}(37.5,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(25,12.5){$b$}
\rput(42.5,12.5){$p_n$}
\rput(12.5,2.5){$b\oDownset$}
\end{pspicture}


==> pictures/fig-claim-h.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Mar 11 21:18:56 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="56.25" y-min="0" y-max="23.38" auto-bounding="true">
%<multicurve fill-color= "#c0c0c0"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 points= "(12.5,5);(12.5,5);(12.5,12.5);(12.5,12.5);(12.5,12.5);(0,5);
%	(0,5);(0,5);(12.5,5)"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(42.5,10)"
%	 p2= "(42.5,15)"
%	 p1= "(27.5,15)"
%	 fill-color= "#f0f0f0"
%	 stroke-width= "0.15"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 points= "(30,5);(30,5);(30,12.5);(30,12.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(56.25,0)"
%	 p2= "(56.25,5)"
%	 p1= "(30,5)"
%	 fill-color= "#f0f0f0"
%	 stroke-width= "0.15"
%	 fill-style= "solid"
%	 />
%<multicurve fill-color= "#dcdcdc"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 points= "(30,5);(30,5);(30,12.5);(30,12.5);(30,12.5);(0,5);
%	(0,5);(0,5);(30,5)"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(30,0)"
%	 p2= "(30,5)"
%	 p1= "(-0,5)"
%	 fill-color= "#f0f0f0"
%	 stroke-width= "0.15"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(21.25,13.75)"
%	 stroke-width= "0.05"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.25,11.25)"
%	 stroke-width= "0.15"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%
%</text>
%<multicurve stroke-width= "0.15"
%	 points= "(30,12.5);(30,12.5);(30,22.5);(30,22.5)"
%	 fill-style= "none"
%	 />
%<circle p3= "(30.63,23.12)"
%	 p2= "(29.37,23.12)"
%	 p1= "(29.37,21.88)"
%	 fill-color= "#ffffff"
%	 stroke-width= "0.15"
%	 closure= "plain"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.15"
%	 points= "(25,2.5);(25,2.5);(30,12.5);(30,12.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.15"
%	 points= "(20,2.5);(20,2.5);(30,12.5);(30,12.5)"
%	 fill-style= "none"
%	 />
%<circle p3= "(25.63,3.12)"
%	 p2= "(24.37,3.12)"
%	 p1= "(24.37,1.88)"
%	 fill-color= "#ffffff"
%	 stroke-width= "0.15"
%	 closure= "plain"
%	 fill-style= "solid"
%	 />
%<circle p3= "(20.63,3.12)"
%	 p2= "(19.37,3.12)"
%	 p1= "(19.37,1.88)"
%	 fill-color= "#ffffff"
%	 stroke-width= "0.15"
%	 closure= "plain"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.12,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$q_1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$a$
%</text>
%<multicurve stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 points= "(0,5);(0,5);(30,12.5);(30,12.5)"
%	 fill-style= "none"
%	 />
%<circle p3= "(13.12,13.12)"
%	 p2= "(11.88,13.12)"
%	 p1= "(11.88,11.88)"
%	 fill-color= "#ffffff"
%	 stroke-width= "0.15"
%	 closure= "plain"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$q_4$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.88,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$q_3$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(36.25,12.5)"
%	 stroke-width= "0.15"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_i$
%</text>
%<parallelogram p3= "(42.5,10)"
%	 p2= "(42.5,15)"
%	 p1= "(27.5,15)"
%	 stroke-width= "0.15"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-color= "#808080"
%	 anchor-point= "(25,13.75)"
%	 stroke-width= "0.05"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$q_2$
%</text>
%<circle p3= "(30.62,13.12)"
%	 p2= "(29.38,13.12)"
%	 p1= "(29.38,11.88)"
%	 fill-color= "#ffffff"
%	 stroke-width= "0.15"
%	 closure= "plain"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(37,19)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$q_3$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(56.25,23.38)
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=lightgray,fillstyle=solid](12.5,5)
(12.5,12.5)
(0,5)(12.5,5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](27.5,15)(42.5,15)(42.5,10)(27.5,10)
\psline[linewidth=0.05,linecolor=gray](30,5)(30,12.5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](30,5)(56.25,5)(56.25,0)(30,0)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](30,5)
(30,12.5)
(0,5)(30,5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.15,fillcolor=userFillColour,fillstyle=solid](-0,5)(30,5)(30,0)(0,0)
\rput(21.25,13.75){}
\rput(31.25,11.25){}
\psline[linewidth=0.15](30,12.5)(30,22.5)
\rput{0}(30,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\psline[linewidth=0.15](25,2.5)(30,12.5)
\psline[linewidth=0.15](20,2.5)(30,12.5)
\rput{0}(25,2.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20,2.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(28.12,2.5){$q_1$}
\rput(17.5,2.5){$a$}
\psline[linewidth=0.05,linecolor=gray](0,5)(30,12.5)
\rput{0}(12.5,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(9.38,13.75){$q_4$}
\rput(26.88,22.5){$q_3$}
\rput(36.25,12.5){$B_i$}
\pspolygon[linewidth=0.15](27.5,15)(42.5,15)(42.5,10)(27.5,10)
\rput(25,13.75){$q_2$}
\rput{0}(30,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(37,19){$q_3$}
\end{pspicture}


==> pictures/fig-jp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Mar 11 23:38:43 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="85" y-min="0" y-max="23.38" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 points= "(0,15);(0,15);(47.5,22.5);(47.5,22.5);(47.5,22.5);(47.5,15);
%	(47.5,15);(47.5,15);(0,15);(0,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#cccccc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(15,10);(15,10);(15,5);(15,5);(15,5);(-0,5);
%	(-0,5);(-0,5);(0,10);(0,10);(0,10);(15,10)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#a0a0a0"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(30,10);(30,10);(30,5);(30,5);(30,5);(0,5);
%	(0,5);(0,5);(15,10);(15,10);(15,10);(30,10)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#b4b4b4"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(57.5,10);(57.5,10);(57.5,5);(57.5,5);(57.5,5);(0,5);
%	(0,5);(0,5);(42.5,10);(42.5,10);(42.5,10);(57.5,10)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#c8c8c8"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(-0,5);(-0,5);(85,5);(85,5);(85,5);(85,0);
%	(85,0);(85,0);(-0,0);(-0,0);(-0,0);(-0,5)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(36.25,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A$
%</text>
%<g>
%<multicurve fill-style= "solid"
%	 points= "(0,15);(0,15);(15,15);(15,15);(15,15);(15,10);
%	(15,10);(15,10);(0,10);(0,10);(0,10);(0,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_1$
%</text>
%</g>
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(15,15);(15,15);(30,15);(30,15);(30,15);(30,10);
%	(30,10);(30,10);(15,10);(15,10);(15,10);(15,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_2$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(42.5,15);(42.5,15);(57.5,15);(57.5,15);(57.5,15);(57.5,10);
%	(57.5,10);(57.5,10);(42.5,10);(42.5,10);(42.5,10);(42.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(53.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_{j(p)}$
%</text>
%<multicurve fill-style= "none"
%	 points= "(47.5,2.5);(47.5,2.5);(47.5,22.5);(47.5,22.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(48.12,3.12)"
%	 p2= "(46.88,3.12)"
%	 p1= "(46.88,1.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(48.12,13.12)"
%	 p2= "(46.88,13.12)"
%	 p1= "(46.88,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(32.5,12.5);(32.5,12.5);(47.5,22.5);(47.5,22.5)"
%	 stroke-width= "0.15"
%	 />
%<circle p3= "(33.12,13.12)"
%	 p2= "(31.88,13.12)"
%	 p1= "(31.88,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(48.12,23.12)"
%	 p2= "(46.88,23.12)"
%	 p1= "(46.88,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$p$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(63.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(70,15);(70,15);(85,15);(85,15);(85,15);(85,10);
%	(85,10);(85,10);(70,10);(70,10);(70,10);(70,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(77.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_0$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(85,23.38)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(47.5,22.5)
(47.5,15)(0,15)
\newrgbcolor{userFillColour}{0.63 0.63 0.63}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](15,10)
(15,5)
(-0,5)
(0,10)(15,10)
\newrgbcolor{userFillColour}{0.71 0.71 0.71}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](30,10)
(30,5)
(0,5)
(15,10)(30,10)
\newrgbcolor{userFillColour}{0.78 0.78 0.78}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](57.5,10)
(57.5,5)
(0,5)
(42.5,10)(57.5,10)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](-0,5)
(85,5)
(85,0)
(-0,0)(-0,5)
\rput(36.25,2.5){$A$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(15,15)
(15,10)
(0,10)(0,15)
\rput(7.5,12.5){$B_1$}
\rput(38.75,12.5){$\ldots$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](15,15)
(30,15)
(30,10)
(15,10)(15,15)
\rput(22.5,12.5){$B_2$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](42.5,15)
(57.5,15)
(57.5,10)
(42.5,10)(42.5,15)
\rput(53.75,12.5){$B_{j(p)}$}
\psline[linewidth=0.2](47.5,2.5)(47.5,22.5)
\rput{0}(47.5,2.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(47.5,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\psline[linewidth=0.15,linestyle=dashed,dash=1 1](32.5,12.5)(47.5,22.5)
\rput{0}(32.5,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(47.5,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(50,22.5){$p$}
\rput(63.75,12.5){$\ldots$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](70,15)
(85,15)
(85,10)
(70,10)(70,15)
\rput(77.5,12.5){$B_0$}
\end{pspicture}


==> pictures/fig-layers.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Mar 17 23:03:08 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="82.5" y-min="0" y-max="32.5" auto-bounding="true">
%<g>
%<g>
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(25,10);(25,10)"
%	 stroke-color= "#404040"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(0,20);(0,20)"
%	 stroke-color= "#404040"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(0,30);(0,30)"
%	 stroke-color= "#404040"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,30);(15,30);(15,10);(15,10)"
%	 stroke-width= "0.2"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(5,10);(5,10);(15,20);(15,20)"
%	 stroke-width= "0.05"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(5,10);(5,10);(15,30);(15,30)"
%	 stroke-width= "0.05"
%	 />
%<circle p3= "(15.62,10.62)"
%	 p2= "(14.38,10.62)"
%	 p1= "(14.38,9.38)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(15.62,20.62)"
%	 p2= "(14.38,20.62)"
%	 p1= "(14.38,19.38)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(15.62,30.62)"
%	 p2= "(14.38,30.62)"
%	 p1= "(14.38,29.38)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(5.62,10.62)"
%	 p2= "(4.38,10.62)"
%	 p1= "(4.38,9.38)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.5,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$L_i$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.75,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$L_{i+1}$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.5,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$L_j$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$\vdots$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,7.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$x$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$y$
%</text>
%</g>
%<multicurve fill-style= "none"
%	 points= "(55,10);(55,10);(80,10);(80,10)"
%	 stroke-color= "#404040"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,20);(80,20);(55,20);(55,20)"
%	 stroke-color= "#404040"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,20);(70,20);(70,10);(70,10)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(70.62,10.62)"
%	 p2= "(69.38,10.62)"
%	 p1= "(69.38,9.38)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(70.62,20.62)"
%	 p2= "(69.38,20.62)"
%	 p1= "(69.38,19.38)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(60.62,10.62)"
%	 p2= "(59.38,10.62)"
%	 p1= "(59.38,9.38)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.5,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$L_i$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.5,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$L_j$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,7.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$x$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.25,16.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "center-h"
%	 >
%$\vdots$
%</text>
%</g>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-1.25,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "left"
%	 >
%(i) \ThreePlusOne is forbidden
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.05"
%	 text-hor-align= "left"
%	 >
%(ii) $x\oDownset \subsetneq y\oDownset \Rightarrow\ x \prec y$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,23)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$y$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(69.38,7.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$z$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(82.5,32.5)
\psline[linewidth=0.05,linecolor=darkgray](0,10)(25,10)
\psline[linewidth=0.05,linecolor=darkgray](25,20)(0,20)
\psline[linewidth=0.05,linecolor=darkgray](25,30)(0,30)
\psline[linewidth=0.2](15,30)(15,10)
\psline[linewidth=0.05,linestyle=dashed,dash=1 1](5,10)(15,20)
\psline[linewidth=0.05,linestyle=dashed,dash=1 1](5,10)(15,30)
\rput{0}(15,10){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(15,20){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(15,30){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(5,10){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(27.5,10){$L_i$}
\rput(28.75,20){$L_{i+1}$}
\rput(27.5,30){$L_j$}
\rput(26.25,26.25){$\vdots$}
\rput(5,7.5){$x$}
\rput(15,32.5){$y$}
\psline[linewidth=0.05,linecolor=darkgray](55,10)(80,10)
\psline[linewidth=0.05,linecolor=darkgray](80,20)(55,20)
\psline[linewidth=0.2](70,20)(70,10)
\rput{0}(70,10){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(70,20){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(60,10){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(82.5,10){$L_i$}
\rput(82.5,20){$L_j$}
\rput(60,7.5){$x$}
\rput(81.25,16.25){$\vdots$}
\rput[l](-1.25,0){(i) \ThreePlusOne is forbidden}
\rput[l](52.5,0){(ii) $x\oDownset \subsetneq y\oDownset \Rightarrow\ x \prec y$}
\rput(70,23){$y$}
\rput(69.38,7.5){$z$}
\end{pspicture}


==> pictures/fig-local-width.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 05 11:21:35 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="90" y-min="0" y-max="26.88" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$r$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(33.75,15);(33.75,15);(45,15);(45,15);(45,15);(45,10);
%	(45,10);(45,10);(33.75,10);(33.75,10);(33.75,10);(33.75,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,15);(33.75,15);(45,15);(45,15);(45,15);(45,10);
%	(45,10);(45,10);(33.75,10);(33.75,10);(33.75,10);(33.75,15)"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,25);(22.5,25);(33.75,25);(33.75,25);(33.75,25);(33.75,20);
%	(33.75,20);(33.75,20);(22.5,20);(22.5,20);(22.5,20);(22.5,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(-0,5);(-0,5);(90,5);(90,5);(90,5);(90,0);
%	(90,0);(90,0);(-0,0);(-0,0);(-0,0);(-0,5)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A$
%</text>
%<circle p3= "(33.12,13.12)"
%	 p2= "(31.88,13.12)"
%	 p1= "(31.88,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(34,20);(34,20);(68,20);(68,20);(68,20);(36,13);
%	(36,13);(36,13);(34,20)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.05"
%	 fill-color= "#cccccc"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.5,26.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$U_{j-1}$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(0,25);(0,25);(11.25,25);(11.25,25);(11.25,25);(11.25,20);
%	(11.25,20);(11.25,20);(0,20);(0,20);(0,20);(0,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(33.75,25);(33.75,25);(45,25);(45,25);(45,25);(45,20);
%	(45,20);(45,20);(33.75,20);(33.75,20);(33.75,20);(33.75,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$U_1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.75,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$U_j$
%</text>
%<circle p3= "(66.87,13.12)"
%	 p2= "(65.63,13.12)"
%	 p1= "(65.63,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(56.25,25);(56.25,25);(67.5,25);(67.5,25);(67.5,25);(67.5,20);
%	(67.5,20);(67.5,20);(56.25,20);(56.25,20);(56.25,20);(56.25,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.25,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$U_k$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(56.25,15);(56.25,15);(67.5,15);(67.5,15);(67.5,15);(67.5,10);
%	(67.5,10);(67.5,10);(56.25,10);(56.25,10);(56.25,10);(56.25,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.25,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_k$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(67.5,15);(67.5,15);(78.75,15);(78.75,15);(78.75,15);(78.75,10);
%	(78.75,10);(78.75,10);(67.5,10);(67.5,10);(67.5,10);(67.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(72.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_{k+1}$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(78.75,15);(78.75,15);(90,15);(90,15);(90,15);(90,10);
%	(90,10);(90,10);(78.75,10);(78.75,10);(78.75,10);(78.75,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(83.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_0$
%</text>
%<multicurve fill-style= "none"
%	 points= "(22.5,25);(22.5,25);(33.75,25);(33.75,25);(33.75,25);(33.75,20);
%	(33.75,20);(33.75,20);(22.5,20);(22.5,20);(22.5,20);(22.5,25)"
%	 stroke-width= "0.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.12,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$r$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(0,15);(0,15);(32,22);(32,22);(32,22);(34,15);
%	(34,15);(34,15);(0,15);(0,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.05"
%	 fill-color= "#cccccc"
%	 />
%<circle p3= "(32.62,22.74)"
%	 p2= "(31.38,22.74)"
%	 p1= "(31.38,21.5)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.75,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$p$
%</text>
%<circle p3= "(36.24,13.11)"
%	 p2= "(35,13.11)"
%	 p1= "(35,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<g>
%<multicurve fill-style= "solid"
%	 points= "(0,15);(0,15);(11.25,15);(11.25,15);(11.25,15);(11.25,10);
%	(11.25,10);(11.25,10);(0,10);(0,10);(0,10);(0,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_1$
%</text>
%</g>
%<multicurve fill-style= "solid"
%	 points= "(22.5,15);(22.5,15);(33.75,15);(33.75,15);(33.75,15);(33.75,10);
%	(33.75,10);(33.75,10);(22.5,10);(22.5,10);(22.5,10);(22.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_{j-1}$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_j$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(90,26.88)
\rput(37.5,12.5){$r$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](33.75,15)
(45,15)
(45,10)
(33.75,10)(33.75,15)
\pspolygon[linewidth=0.05](33.75,15)
(45,15)
(45,10)
(33.75,10)(33.75,15)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](22.5,25)
(33.75,25)
(33.75,20)
(22.5,20)(22.5,25)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](-0,5)
(90,5)
(90,0)
(-0,0)(-0,5)
\rput(44.38,2.5){$A$}
\rput{0}(32.5,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(16.25,12.5){$\ldots$}
\rput(16.25,22.5){$\ldots$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\pspolygon[linewidth=0.05,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](34,20)
(68,20)
(36,13)(34,20)
\rput(27.5,26.88){$U_{j-1}$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,25)
(11.25,25)
(11.25,20)
(0,20)(0,25)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](33.75,25)
(45,25)
(45,20)
(33.75,20)(33.75,25)
\rput(5,22.5){$U_1$}
\rput(38.75,22.5){$U_j$}
\rput{0}(66.25,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(50,12.5){$\ldots$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](56.25,25)
(67.5,25)
(67.5,20)
(56.25,20)(56.25,25)
\rput(50,22.5){$\ldots$}
\rput(61.25,22.5){$U_k$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](56.25,15)
(67.5,15)
(67.5,10)
(56.25,10)(56.25,15)
\rput(61.25,12.5){$B_k$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](67.5,15)
(78.75,15)
(78.75,10)
(67.5,10)(67.5,15)
\rput(72.5,12.5){$B_{k+1}$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](78.75,15)
(90,15)
(90,10)
(78.75,10)(78.75,15)
\rput(83.75,12.5){$B_0$}
\pspolygon[linewidth=0.05](22.5,25)
(33.75,25)
(33.75,20)
(22.5,20)(22.5,25)
\rput(38.12,12.5){$r$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[linewidth=0.05,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,15)
(32,22)
(34,15)(0,15)
\rput{0}(32,22.12){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(28.75,22.5){$p$}
\rput{0}(35.62,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(11.25,15)
(11.25,10)
(0,10)(0,15)
\rput(5,12.5){$B_1$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](22.5,15)
(33.75,15)
(33.75,10)
(22.5,10)(22.5,15)
\rput(27.5,12.5){$B_{j-1}$}
\rput(42.5,12.5){$B_j$}
\end{pspicture}


==> pictures/fig-lower-bound-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Feb 09 18:00:42 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="108.75" y-min="0" y-max="15" auto-bounding="true">
%<parallelogram stroke-width= "0.05"
%	 p3= "(41.25,5)"
%	 p2= "(41.25,10)"
%	 p1= "(0,10)"
%	 stroke-color= "#808080"
%	 fill-color= "#dcdcdc"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(108.75,10);(108.75,10);(108.75,5);(108.75,5);(108.75,5);(0,5);
%	(0,5);(0,5);(68.12,10);(68.12,10);(68.12,10);(108.75,10)"
%	 fill-color= "#dcdcdc"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(41.25,4.38);(41.25,4.38);(41.25,9.38);(41.25,9.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(41.25,5);(41.25,5);(108.75,5);(108.75,5);(108.75,5);(108.75,0);
%	(108.75,0);(108.75,0);(41.25,0);(41.25,0);(41.25,0);(41.25,5)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(43.57,3.07)"
%	 p2= "(42.33,3.07)"
%	 p1= "(42.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(46.77,3.07)"
%	 p2= "(45.53,3.07)"
%	 p1= "(45.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(49.97,3.07)"
%	 p2= "(48.73,3.07)"
%	 p1= "(48.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(53.17,3.07)"
%	 p2= "(51.93,3.07)"
%	 p1= "(51.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(56.37,3.07)"
%	 p2= "(55.13,3.07)"
%	 p1= "(55.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(59.57,3.07)"
%	 p2= "(58.33,3.07)"
%	 p1= "(58.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(62.77,3.07)"
%	 p2= "(61.53,3.07)"
%	 p1= "(61.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(65.97,3.07)"
%	 p2= "(64.73,3.07)"
%	 p1= "(64.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(69.17,3.07)"
%	 p2= "(67.93,3.07)"
%	 p1= "(67.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(72.37,3.07)"
%	 p2= "(71.13,3.07)"
%	 p1= "(71.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(75.57,3.07)"
%	 p2= "(74.33,3.07)"
%	 p1= "(74.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(78.77,3.07)"
%	 p2= "(77.53,3.07)"
%	 p1= "(77.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(81.97,3.07)"
%	 p2= "(80.73,3.07)"
%	 p1= "(80.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(85.17,3.07)"
%	 p2= "(83.93,3.07)"
%	 p1= "(83.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(88.37,3.07)"
%	 p2= "(87.13,3.07)"
%	 p1= "(87.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(91.57,3.07)"
%	 p2= "(90.33,3.07)"
%	 p1= "(90.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(94.77,3.07)"
%	 p2= "(93.53,3.07)"
%	 p1= "(93.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(97.97,3.07)"
%	 p2= "(96.73,3.07)"
%	 p1= "(96.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(101.17,3.07)"
%	 p2= "(99.93,3.07)"
%	 p1= "(99.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(104.37,3.07)"
%	 p2= "(103.13,3.07)"
%	 p1= "(103.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(107.57,3.07)"
%	 p2= "(106.33,3.07)"
%	 p1= "(106.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(67.5,15);(67.5,15);(108.75,15);(108.75,15);(108.75,15);(108.75,10);
%	(108.75,10);(108.75,10);(67.5,10);(67.5,10);(67.5,10);(67.5,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(69.47,13.07)"
%	 p2= "(68.23,13.07)"
%	 p1= "(68.23,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(72.67,13.07)"
%	 p2= "(71.43,13.07)"
%	 p1= "(71.43,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(75.87,13.07)"
%	 p2= "(74.63,13.07)"
%	 p1= "(74.63,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(79.07,13.07)"
%	 p2= "(77.83,13.07)"
%	 p1= "(77.83,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(82.27,13.07)"
%	 p2= "(81.03,13.07)"
%	 p1= "(81.03,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(85.47,13.07)"
%	 p2= "(84.23,13.07)"
%	 p1= "(84.23,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(88.67,13.07)"
%	 p2= "(87.43,13.07)"
%	 p1= "(87.43,11.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(91.87,13.07)"
%	 p2= "(90.63,13.07)"
%	 p1= "(90.63,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(95.07,13.07)"
%	 p2= "(93.83,13.07)"
%	 p1= "(93.83,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(98.27,13.07)"
%	 p2= "(97.03,13.07)"
%	 p1= "(97.03,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(101.47,13.07)"
%	 p2= "(100.23,13.07)"
%	 p1= "(100.23,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(104.67,13.07)"
%	 p2= "(103.43,13.07)"
%	 p1= "(103.43,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(107.87,13.07)"
%	 p2= "(106.63,13.07)"
%	 p1= "(106.63,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(88.13,12.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_0$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(0,15);(0,15);(41.25,15);(41.25,15);(41.25,15);(41.25,10);
%	(41.25,10);(41.25,10);(0,10);(0,10);(0,10);(0,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(1.97,13.07)"
%	 p2= "(0.73,13.07)"
%	 p1= "(0.73,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(5.17,13.07)"
%	 p2= "(3.93,13.07)"
%	 p1= "(3.93,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(8.37,13.07)"
%	 p2= "(7.13,13.07)"
%	 p1= "(7.13,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(11.57,13.07)"
%	 p2= "(10.33,13.07)"
%	 p1= "(10.33,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(14.77,13.07)"
%	 p2= "(13.53,13.07)"
%	 p1= "(13.53,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(17.97,13.07)"
%	 p2= "(16.73,13.07)"
%	 p1= "(16.73,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(21.17,13.07)"
%	 p2= "(19.93,13.07)"
%	 p1= "(19.93,11.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(24.37,13.07)"
%	 p2= "(23.13,13.07)"
%	 p1= "(23.13,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(27.57,13.07)"
%	 p2= "(26.33,13.07)"
%	 p1= "(26.33,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(30.77,13.07)"
%	 p2= "(29.53,13.07)"
%	 p1= "(29.53,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(33.97,13.07)"
%	 p2= "(32.73,13.07)"
%	 p1= "(32.73,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(37.17,13.07)"
%	 p2= "(35.93,13.07)"
%	 p1= "(35.93,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(40.37,13.07)"
%	 p2= "(39.13,13.07)"
%	 p1= "(39.13,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20.63,12.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_1$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(0,5);(0,5);(41.25,5);(41.25,5);(41.25,5);(41.25,0);
%	(41.25,0);(41.25,0);(0,0);(0,0);(0,0);(0,5)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(1.97,3.07)"
%	 p2= "(0.73,3.07)"
%	 p1= "(0.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(5.17,3.07)"
%	 p2= "(3.93,3.07)"
%	 p1= "(3.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(8.37,3.07)"
%	 p2= "(7.13,3.07)"
%	 p1= "(7.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(11.57,3.07)"
%	 p2= "(10.33,3.07)"
%	 p1= "(10.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(14.77,3.07)"
%	 p2= "(13.53,3.07)"
%	 p1= "(13.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(17.97,3.07)"
%	 p2= "(16.73,3.07)"
%	 p1= "(16.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(21.17,3.07)"
%	 p2= "(19.93,3.07)"
%	 p1= "(19.93,1.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(24.37,3.07)"
%	 p2= "(23.13,3.07)"
%	 p1= "(23.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(27.57,3.07)"
%	 p2= "(26.33,3.07)"
%	 p1= "(26.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(30.77,3.07)"
%	 p2= "(29.53,3.07)"
%	 p1= "(29.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(33.97,3.07)"
%	 p2= "(32.73,3.07)"
%	 p1= "(32.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(37.17,3.07)"
%	 p2= "(35.93,3.07)"
%	 p1= "(35.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(40.37,3.07)"
%	 p2= "(39.13,3.07)"
%	 p1= "(39.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20.63,2.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$A_0$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(108.75,15)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](0,10)(41.25,10)(41.25,5)(0,5)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](108.75,10)
(108.75,5)
(0,5)
(68.12,10)(108.75,10)
\psline[linewidth=0.05,linecolor=gray](41.25,4.38)(41.25,9.38)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](41.25,5)
(108.75,5)
(108.75,0)
(41.25,0)(41.25,5)
\rput{0}(42.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(46.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(49.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(52.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(58.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(62.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(65.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(68.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(71.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(74.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(78.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(81.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(84.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(87.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(90.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(94.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(97.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(103.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(106.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](67.5,15)
(108.75,15)
(108.75,10)
(67.5,10)(67.5,15)
\rput{0}(68.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(72.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(75.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(78.45,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(81.65,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(84.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(88.05,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(91.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(94.45,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(97.65,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(104.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(107.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(88.13,12.38){$B_0$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(41.25,15)
(41.25,10)
(0,10)(0,15)
\rput{0}(1.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(23.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(26.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(20.63,12.38){$B_1$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,5)
(41.25,5)
(41.25,0)
(0,0)(0,5)
\rput{90}(1.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,2.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(23.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(26.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(20.63,2.38){$A_0$}
\end{pspicture}


==> pictures/fig-lower-bound-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Feb 09 18:03:14 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="108.75" y-min="0" y-max="25" auto-bounding="true">
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(41.25,10);(41.25,10);(57.5,10);(57.5,10);(57.5,10);(57.5,5);
%	(57.5,5);(57.5,5);(0,5);(0,5);(0,5);(41.25,10)"
%	 fill-color= "#dcdcdc"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(0,20);(0,20);(15.63,20);(15.63,20);(15.63,20);(15.63,15);
%	(15.63,15);(15.63,15);(0,15);(0,15);(0,15);(0,20)"
%	 fill-color= "#dcdcdc"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(41.25,20);(41.25,20);(41.25,15);(41.25,15);(41.25,15);(0,15);
%	(0,15);(0,15);(25.62,20);(25.62,20);(25.62,20);(41.25,20)"
%	 fill-color= "#dcdcdc"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(15.63,20);(15.63,20);(15.63,15);(15.63,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(41.25,5);(41.25,5);(108.75,5);(108.75,5);(108.75,5);(108.75,0);
%	(108.75,0);(108.75,0);(41.25,0);(41.25,0);(41.25,0);(41.25,5)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(41.25,5);(41.25,5);(57.5,5);(57.5,5);(57.5,5);(57.5,0);
%	(57.5,0);(57.5,0);(41.25,0);(41.25,0);(41.25,0);(41.25,5)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(0,5);(0,5);(41.25,5);(41.25,5);(41.25,5);(41.25,0);
%	(41.25,0);(41.25,0);(0,0);(0,0);(0,0);(0,5)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(41.25,15);(41.25,15);(57.5,15);(57.5,15);(57.5,15);(57.5,10);
%	(57.5,10);(57.5,10);(41.25,10);(41.25,10);(41.25,10);(41.25,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(0,15);(0,15);(41.25,15);(41.25,15);(41.25,15);(41.25,10);
%	(41.25,10);(41.25,10);(0,10);(0,10);(0,10);(0,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(1.97,3.07)"
%	 p2= "(0.73,3.07)"
%	 p1= "(0.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(5.17,3.07)"
%	 p2= "(3.93,3.07)"
%	 p1= "(3.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(8.37,3.07)"
%	 p2= "(7.13,3.07)"
%	 p1= "(7.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(11.57,3.07)"
%	 p2= "(10.33,3.07)"
%	 p1= "(10.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(14.77,3.07)"
%	 p2= "(13.53,3.07)"
%	 p1= "(13.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(17.97,3.07)"
%	 p2= "(16.73,3.07)"
%	 p1= "(16.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(21.17,3.07)"
%	 p2= "(19.93,3.07)"
%	 p1= "(19.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(24.37,3.07)"
%	 p2= "(23.13,3.07)"
%	 p1= "(23.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(27.57,3.07)"
%	 p2= "(26.33,3.07)"
%	 p1= "(26.33,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(30.77,3.07)"
%	 p2= "(29.53,3.07)"
%	 p1= "(29.53,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(33.97,3.07)"
%	 p2= "(32.73,3.07)"
%	 p1= "(32.73,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(37.17,3.07)"
%	 p2= "(35.93,3.07)"
%	 p1= "(35.93,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(40.37,3.07)"
%	 p2= "(39.13,3.07)"
%	 p1= "(39.13,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(17.97,23.07)"
%	 p2= "(16.73,23.07)"
%	 p1= "(16.73,21.83)"
%	 stroke-color= "#ffffff"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(21.17,23.07)"
%	 p2= "(19.93,23.07)"
%	 p1= "(19.93,21.83)"
%	 stroke-color= "#ffffff"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(24.37,23.07)"
%	 p2= "(23.13,23.07)"
%	 p1= "(23.13,21.83)"
%	 stroke-color= "#ffffff"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(17.97,13.07)"
%	 p2= "(16.73,13.07)"
%	 p1= "(16.73,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(21.17,13.07)"
%	 p2= "(19.93,13.07)"
%	 p1= "(19.93,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(24.37,13.07)"
%	 p2= "(23.13,13.07)"
%	 p1= "(23.13,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(27.57,13.07)"
%	 p2= "(26.33,13.07)"
%	 p1= "(26.33,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(30.77,13.07)"
%	 p2= "(29.53,13.07)"
%	 p1= "(29.53,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(33.97,13.07)"
%	 p2= "(32.73,13.07)"
%	 p1= "(32.73,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(37.17,13.07)"
%	 p2= "(35.93,13.07)"
%	 p1= "(35.93,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(40.37,13.07)"
%	 p2= "(39.13,13.07)"
%	 p1= "(39.13,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(0,15);(0,15);(15.62,15);(15.62,15);(15.62,15);(15.62,10);
%	(15.62,10);(15.62,10);(0,10);(0,10);(0,10);(0,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(1.97,13.07)"
%	 p2= "(0.73,13.07)"
%	 p1= "(0.73,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(5.17,13.07)"
%	 p2= "(3.93,13.07)"
%	 p1= "(3.93,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(8.37,13.07)"
%	 p2= "(7.13,13.07)"
%	 p1= "(7.13,11.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(14.77,13.07)"
%	 p2= "(13.53,13.07)"
%	 p1= "(13.53,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(11.57,13.07)"
%	 p2= "(10.33,13.07)"
%	 p1= "(10.33,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_1^0$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(0,25);(0,25);(15.62,25);(15.62,25);(15.62,25);(15.62,20);
%	(15.62,20);(15.62,20);(0,20);(0,20);(0,20);(0,25)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(1.97,23.07)"
%	 p2= "(0.73,23.07)"
%	 p1= "(0.73,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(5.17,23.07)"
%	 p2= "(3.93,23.07)"
%	 p1= "(3.93,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(8.37,23.07)"
%	 p2= "(7.13,23.07)"
%	 p1= "(7.13,21.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(14.77,23.07)"
%	 p2= "(13.53,23.07)"
%	 p1= "(13.53,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(11.57,23.07)"
%	 p2= "(10.33,23.07)"
%	 p1= "(10.33,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(8,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$C_1^1$
%</text>
%<circle stroke-width= "0.15"
%	 p3= "(43.57,13.07)"
%	 p2= "(42.33,13.07)"
%	 p1= "(42.33,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(46.77,13.07)"
%	 p2= "(45.53,13.07)"
%	 p1= "(45.53,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(49.97,13.07)"
%	 p2= "(48.73,13.07)"
%	 p1= "(48.73,11.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(53.17,13.07)"
%	 p2= "(51.93,13.07)"
%	 p1= "(51.93,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(56.37,13.07)"
%	 p2= "(55.13,13.07)"
%	 p1= "(55.13,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<g>
%<multicurve stroke-width= "0.05"
%	 points= "(25.62,25);(25.62,25);(41.25,25);(41.25,25);(41.25,25);(41.25,20);
%	(41.25,20);(41.25,20);(25.62,20);(25.62,20);(25.62,20);(25.62,25)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(27.57,23.07)"
%	 p2= "(26.33,23.07)"
%	 p1= "(26.33,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(30.77,23.07)"
%	 p2= "(29.53,23.07)"
%	 p1= "(29.53,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(33.97,23.07)"
%	 p2= "(32.73,23.07)"
%	 p1= "(32.73,21.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(37.17,23.07)"
%	 p2= "(35.93,23.07)"
%	 p1= "(35.93,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(40.37,23.07)"
%	 p2= "(39.13,23.07)"
%	 p1= "(39.13,21.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(33.75,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$C_1^0$
%</text>
%</g>
%<circle stroke-width= "0.15"
%	 p3= "(27.57,13.07)"
%	 p2= "(26.33,13.07)"
%	 p1= "(26.33,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(30.77,13.07)"
%	 p2= "(29.53,13.07)"
%	 p1= "(29.53,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(33.97,13.07)"
%	 p2= "(32.73,13.07)"
%	 p1= "(32.73,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(37.17,13.07)"
%	 p2= "(35.93,13.07)"
%	 p1= "(35.93,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(40.37,13.07)"
%	 p2= "(39.13,13.07)"
%	 p1= "(39.13,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(49,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_2$
%</text>
%<circle stroke-width= "0.15"
%	 p3= "(59.49,3.07)"
%	 p2= "(58.25,3.07)"
%	 p1= "(58.25,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(62.69,3.07)"
%	 p2= "(61.45,3.07)"
%	 p1= "(61.45,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(65.89,3.07)"
%	 p2= "(64.65,3.07)"
%	 p1= "(64.65,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(69.09,3.07)"
%	 p2= "(67.85,3.07)"
%	 p1= "(67.85,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(72.29,3.07)"
%	 p2= "(71.05,3.07)"
%	 p1= "(71.05,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(75.49,3.07)"
%	 p2= "(74.25,3.07)"
%	 p1= "(74.25,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(78.69,3.07)"
%	 p2= "(77.45,3.07)"
%	 p1= "(77.45,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(81.89,3.07)"
%	 p2= "(80.65,3.07)"
%	 p1= "(80.65,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(85.09,3.07)"
%	 p2= "(83.85,3.07)"
%	 p1= "(83.85,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(88.29,3.07)"
%	 p2= "(87.05,3.07)"
%	 p1= "(87.05,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(91.49,3.07)"
%	 p2= "(90.25,3.07)"
%	 p1= "(90.25,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(94.69,3.07)"
%	 p2= "(93.45,3.07)"
%	 p1= "(93.45,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(97.89,3.07)"
%	 p2= "(96.65,3.07)"
%	 p1= "(96.65,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(101.09,3.07)"
%	 p2= "(99.85,3.07)"
%	 p1= "(99.85,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(104.29,3.07)"
%	 p2= "(103.05,3.07)"
%	 p1= "(103.05,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(107.49,3.07)"
%	 p2= "(106.25,3.07)"
%	 p1= "(106.25,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(43.49,3.07)"
%	 p2= "(42.25,3.07)"
%	 p1= "(42.25,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(46.69,3.07)"
%	 p2= "(45.45,3.07)"
%	 p1= "(45.45,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(49.89,3.07)"
%	 p2= "(48.65,3.07)"
%	 p1= "(48.65,1.83)"
%	 stroke-color= "#808080"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(53.09,3.07)"
%	 p2= "(51.85,3.07)"
%	 p1= "(51.85,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(56.29,3.07)"
%	 p2= "(55.05,3.07)"
%	 p1= "(55.05,1.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(49.38,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$A_1$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(67.5,15);(67.5,15);(108.75,15);(108.75,15);(108.75,15);(108.75,10);
%	(108.75,10);(108.75,10);(67.5,10);(67.5,10);(67.5,10);(67.5,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(69.47,13.07)"
%	 p2= "(68.23,13.07)"
%	 p1= "(68.23,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(72.67,13.07)"
%	 p2= "(71.43,13.07)"
%	 p1= "(71.43,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(75.87,13.07)"
%	 p2= "(74.63,13.07)"
%	 p1= "(74.63,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(79.07,13.07)"
%	 p2= "(77.83,13.07)"
%	 p1= "(77.83,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(82.27,13.07)"
%	 p2= "(81.03,13.07)"
%	 p1= "(81.03,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(85.47,13.07)"
%	 p2= "(84.23,13.07)"
%	 p1= "(84.23,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(88.67,13.07)"
%	 p2= "(87.43,13.07)"
%	 p1= "(87.43,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(91.87,13.07)"
%	 p2= "(90.63,13.07)"
%	 p1= "(90.63,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(95.07,13.07)"
%	 p2= "(93.83,13.07)"
%	 p1= "(93.83,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(98.27,13.07)"
%	 p2= "(97.03,13.07)"
%	 p1= "(97.03,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(101.47,13.07)"
%	 p2= "(100.23,13.07)"
%	 p1= "(100.23,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(104.67,13.07)"
%	 p2= "(103.43,13.07)"
%	 p1= "(103.43,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%<circle stroke-width= "0.15"
%	 p3= "(107.87,13.07)"
%	 p2= "(106.63,13.07)"
%	 p1= "(106.63,11.83)"
%	 closure= "plain"
%	 fill-color= "#ffffff"
%	 fill-style= "solid"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(108.75,25)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](41.25,10)
(57.5,10)
(57.5,5)
(0,5)(41.25,10)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](0,20)
(15.63,20)
(15.63,15)
(0,15)(0,20)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](41.25,20)
(41.25,15)
(0,15)
(25.62,20)(41.25,20)
\psline[linewidth=0.05,linecolor=gray](15.63,20)(15.63,15)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](41.25,5)
(108.75,5)
(108.75,0)
(41.25,0)(41.25,5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](41.25,5)
(57.5,5)
(57.5,0)
(41.25,0)(41.25,5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,5)
(41.25,5)
(41.25,0)
(0,0)(0,5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](41.25,15)
(57.5,15)
(57.5,10)
(41.25,10)(41.25,15)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(41.25,15)
(41.25,10)
(0,10)(0,15)
\rput{90}(1.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(23.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(26.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.35,22.45){\psellipse[linewidth=0.15,linecolor=white,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,22.45){\psellipse[linewidth=0.15,linecolor=white,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(23.75,22.45){\psellipse[linewidth=0.15,linecolor=white,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(23.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(26.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(15.62,15)
(15.62,10)
(0,10)(0,15)
\rput{0}(1.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(7.5,12.5){$B_1^0$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,25)
(15.62,25)
(15.62,20)
(0,20)(0,25)
\rput{0}(1.35,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(8,22.5){$C_1^1$}
\rput{0}(42.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(46.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(49.35,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(52.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](25.62,25)
(41.25,25)
(41.25,20)
(25.62,20)(25.62,25)
\rput{0}(26.95,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(33.75,22.5){$C_1^0$}
\rput{0}(26.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(49,12.5){$B_2$}
\rput{0}(58.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(62.07,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(65.27,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(68.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(71.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(74.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(78.07,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(81.27,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(84.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(87.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(90.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(94.07,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(97.27,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(103.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(106.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(42.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(46.07,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(49.27,2.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(52.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(49.38,2.5){$A_1$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](67.5,15)
(108.75,15)
(108.75,10)
(67.5,10)(67.5,15)
\rput{0}(68.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(72.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(75.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(78.45,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(81.65,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(84.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(88.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(91.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(94.45,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(97.65,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(104.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(107.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\end{pspicture}


==> pictures/fig-lower-bound-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Feb 29 23:46:32 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="108.75" y-min="0" y-max="25" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 points= "(57.5,10);(57.5,10);(63.75,10);(63.75,10);(63.75,10);(63.75,5);
%	(63.75,5);(63.75,5);(0,5);(0,5);(0,5);(57.5,10)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#dcdcdc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(15.62,20);(15.62,20);(21.88,20);(21.88,20);(21.88,20);(21.88,15);
%	(21.88,15);(21.88,15);(0,15);(0,15);(0,15);(15.62,20)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#dcdcdc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(47.5,20);(47.5,20);(47.5,15);(47.5,15);(47.5,15);(0,15);
%	(0,15);(0,15);(41.25,20);(41.25,20);(41.25,20);(47.5,20)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#dcdcdc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(57.5,20);(57.5,20);(57.5,15);(57.5,15);(57.5,15);(0,15);
%	(0,15);(0,15);(51.25,20);(51.25,20);(51.25,20);(57.5,20)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#dcdcdc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(57.5,5);(57.5,5);(63.75,5);(63.75,5);(63.75,5);(63.75,0);
%	(63.75,0);(63.75,0);(57.5,0);(57.5,0);(57.5,0);(57.5,5)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(0,5);(0,5);(57.5,5);(57.5,5);(57.5,5);(57.5,0);
%	(57.5,0);(57.5,0);(0,0);(0,0);(0,0);(0,5)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(63.75,5);(63.75,5);(108.75,5);(108.75,5);(108.75,5);(108.75,0);
%	(108.75,0);(108.75,0);(63.75,0);(63.75,0);(63.75,0);(63.75,5)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(1.97,3.07)"
%	 p2= "(0.73,3.07)"
%	 p1= "(0.73,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(5.17,3.07)"
%	 p2= "(3.93,3.07)"
%	 p1= "(3.93,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(8.37,3.07)"
%	 p2= "(7.13,3.07)"
%	 p1= "(7.13,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(11.57,3.07)"
%	 p2= "(10.33,3.07)"
%	 p1= "(10.33,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(14.77,3.07)"
%	 p2= "(13.53,3.07)"
%	 p1= "(13.53,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(17.97,3.07)"
%	 p2= "(16.73,3.07)"
%	 p1= "(16.73,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(21.17,3.07)"
%	 p2= "(19.93,3.07)"
%	 p1= "(19.93,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(24.37,3.07)"
%	 p2= "(23.13,3.07)"
%	 p1= "(23.13,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(27.57,3.07)"
%	 p2= "(26.33,3.07)"
%	 p1= "(26.33,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(30.77,3.07)"
%	 p2= "(29.53,3.07)"
%	 p1= "(29.53,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(33.97,3.07)"
%	 p2= "(32.73,3.07)"
%	 p1= "(32.73,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(37.17,3.07)"
%	 p2= "(35.93,3.07)"
%	 p1= "(35.93,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(40.37,3.07)"
%	 p2= "(39.13,3.07)"
%	 p1= "(39.13,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(67.5,15);(67.5,15);(108.75,15);(108.75,15);(108.75,15);(108.75,10);
%	(108.75,10);(108.75,10);(67.5,10);(67.5,10);(67.5,10);(67.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(69.47,13.07)"
%	 p2= "(68.23,13.07)"
%	 p1= "(68.23,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(72.67,13.07)"
%	 p2= "(71.43,13.07)"
%	 p1= "(71.43,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(75.87,13.07)"
%	 p2= "(74.63,13.07)"
%	 p1= "(74.63,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(79.07,13.07)"
%	 p2= "(77.83,13.07)"
%	 p1= "(77.83,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(82.27,13.07)"
%	 p2= "(81.03,13.07)"
%	 p1= "(81.03,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(85.47,13.07)"
%	 p2= "(84.23,13.07)"
%	 p1= "(84.23,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(88.67,13.07)"
%	 p2= "(87.43,13.07)"
%	 p1= "(87.43,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(91.87,13.07)"
%	 p2= "(90.63,13.07)"
%	 p1= "(90.63,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(95.07,13.07)"
%	 p2= "(93.83,13.07)"
%	 p1= "(93.83,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(98.27,13.07)"
%	 p2= "(97.03,13.07)"
%	 p1= "(97.03,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(101.47,13.07)"
%	 p2= "(100.23,13.07)"
%	 p1= "(100.23,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(104.67,13.07)"
%	 p2= "(103.43,13.07)"
%	 p1= "(103.43,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(107.87,13.07)"
%	 p2= "(106.63,13.07)"
%	 p1= "(106.63,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(59.49,3.07)"
%	 p2= "(58.25,3.07)"
%	 p1= "(58.25,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(62.69,3.07)"
%	 p2= "(61.45,3.07)"
%	 p1= "(61.45,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(65.89,3.07)"
%	 p2= "(64.65,3.07)"
%	 p1= "(64.65,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(69.09,3.07)"
%	 p2= "(67.85,3.07)"
%	 p1= "(67.85,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(72.29,3.07)"
%	 p2= "(71.05,3.07)"
%	 p1= "(71.05,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(75.49,3.07)"
%	 p2= "(74.25,3.07)"
%	 p1= "(74.25,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(78.69,3.07)"
%	 p2= "(77.45,3.07)"
%	 p1= "(77.45,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(81.89,3.07)"
%	 p2= "(80.65,3.07)"
%	 p1= "(80.65,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(85.09,3.07)"
%	 p2= "(83.85,3.07)"
%	 p1= "(83.85,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(88.29,3.07)"
%	 p2= "(87.05,3.07)"
%	 p1= "(87.05,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(91.49,3.07)"
%	 p2= "(90.25,3.07)"
%	 p1= "(90.25,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(94.69,3.07)"
%	 p2= "(93.45,3.07)"
%	 p1= "(93.45,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(97.89,3.07)"
%	 p2= "(96.65,3.07)"
%	 p1= "(96.65,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(101.09,3.07)"
%	 p2= "(99.85,3.07)"
%	 p1= "(99.85,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(104.29,3.07)"
%	 p2= "(103.05,3.07)"
%	 p1= "(103.05,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(107.49,3.07)"
%	 p2= "(106.25,3.07)"
%	 p1= "(106.25,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(43.49,3.07)"
%	 p2= "(42.25,3.07)"
%	 p1= "(42.25,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(46.69,3.07)"
%	 p2= "(45.45,3.07)"
%	 p1= "(45.45,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(49.89,3.07)"
%	 p2= "(48.65,3.07)"
%	 p1= "(48.65,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(53.09,3.07)"
%	 p2= "(51.85,3.07)"
%	 p1= "(51.85,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(56.29,3.07)"
%	 p2= "(55.05,3.07)"
%	 p1= "(55.05,1.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,20);(47.5,20);(47.5,15);(47.5,15)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.88,20);(21.88,20);(21.88,15);(21.88,15)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(41.25,25);(41.25,25);(47.5,25);(47.5,25);(47.5,25);(47.5,20);
%	(47.5,20);(47.5,20);(41.25,20);(41.25,20);(41.25,20);(41.25,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(15.62,25);(15.62,25);(21.88,25);(21.88,25);(21.88,25);(21.88,20);
%	(21.88,20);(21.88,20);(15.62,20);(15.62,20);(15.62,20);(15.62,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(17.97,23.07)"
%	 p2= "(16.73,23.07)"
%	 p1= "(16.73,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(21.17,23.07)"
%	 p2= "(19.93,23.07)"
%	 p1= "(19.93,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(0,25);(0,25);(15.62,25);(15.62,25);(15.62,25);(15.62,20);
%	(15.62,20);(15.62,20);(0,20);(0,20);(0,20);(0,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(1.97,23.07)"
%	 p2= "(0.73,23.07)"
%	 p1= "(0.73,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(5.17,23.07)"
%	 p2= "(3.93,23.07)"
%	 p1= "(3.93,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(8.37,23.07)"
%	 p2= "(7.13,23.07)"
%	 p1= "(7.13,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(14.77,23.07)"
%	 p2= "(13.53,23.07)"
%	 p1= "(13.53,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(11.57,23.07)"
%	 p2= "(10.33,23.07)"
%	 p1= "(10.33,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(25.62,25);(25.62,25);(41.25,25);(41.25,25);(41.25,25);(41.25,20);
%	(41.25,20);(41.25,20);(25.62,20);(25.62,20);(25.62,20);(25.62,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(27.57,23.07)"
%	 p2= "(26.33,23.07)"
%	 p1= "(26.33,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(30.77,23.07)"
%	 p2= "(29.53,23.07)"
%	 p1= "(29.53,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(33.97,23.07)"
%	 p2= "(32.73,23.07)"
%	 p1= "(32.73,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(37.17,23.07)"
%	 p2= "(35.93,23.07)"
%	 p1= "(35.93,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(40.37,23.07)"
%	 p2= "(39.13,23.07)"
%	 p1= "(39.13,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(43.57,23.07)"
%	 p2= "(42.33,23.07)"
%	 p1= "(42.33,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(46.77,23.07)"
%	 p2= "(45.53,23.07)"
%	 p1= "(45.53,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(49.97,23.07)"
%	 p2= "(48.73,23.07)"
%	 p1= "(48.73,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#ffffff"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<g>
%<multicurve fill-style= "solid"
%	 points= "(51.25,25);(51.25,25);(57.5,25);(57.5,25);(57.5,25);(57.5,20);
%	(57.5,20);(57.5,20);(51.25,20);(51.25,20);(51.25,20);(51.25,25)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(53.17,23.07)"
%	 p2= "(51.93,23.07)"
%	 p1= "(51.93,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(56.37,23.07)"
%	 p2= "(55.13,23.07)"
%	 p1= "(55.13,21.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%</g>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$C_2^0$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.7,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$C_2^1$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(0,15);(0,15);(57.5,15);(57.5,15);(57.5,15);(57.5,10);
%	(57.5,10);(57.5,10);(0,10);(0,10);(0,10);(0,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(17.97,13.07)"
%	 p2= "(16.73,13.07)"
%	 p1= "(16.73,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(21.17,13.07)"
%	 p2= "(19.93,13.07)"
%	 p1= "(19.93,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(24.37,13.07)"
%	 p2= "(23.13,13.07)"
%	 p1= "(23.13,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(27.57,13.07)"
%	 p2= "(26.33,13.07)"
%	 p1= "(26.33,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(30.77,13.07)"
%	 p2= "(29.53,13.07)"
%	 p1= "(29.53,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(33.97,13.07)"
%	 p2= "(32.73,13.07)"
%	 p1= "(32.73,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(37.17,13.07)"
%	 p2= "(35.93,13.07)"
%	 p1= "(35.93,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(40.37,13.07)"
%	 p2= "(39.13,13.07)"
%	 p1= "(39.13,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(1.97,13.07)"
%	 p2= "(0.73,13.07)"
%	 p1= "(0.73,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(5.17,13.07)"
%	 p2= "(3.93,13.07)"
%	 p1= "(3.93,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(8.37,13.07)"
%	 p2= "(7.13,13.07)"
%	 p1= "(7.13,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(14.77,13.07)"
%	 p2= "(13.53,13.07)"
%	 p1= "(13.53,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(11.57,13.07)"
%	 p2= "(10.33,13.07)"
%	 p1= "(10.33,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(27.57,13.07)"
%	 p2= "(26.33,13.07)"
%	 p1= "(26.33,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(30.77,13.07)"
%	 p2= "(29.53,13.07)"
%	 p1= "(29.53,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(33.97,13.07)"
%	 p2= "(32.73,13.07)"
%	 p1= "(32.73,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(37.17,13.07)"
%	 p2= "(35.93,13.07)"
%	 p1= "(35.93,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(40.37,13.07)"
%	 p2= "(39.13,13.07)"
%	 p1= "(39.13,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<g>
%<multicurve fill-style= "solid"
%	 points= "(57.5,15);(57.5,15);(63.75,15);(63.75,15);(63.75,15);(63.75,10);
%	(63.75,10);(63.75,10);(57.5,10);(57.5,10);(57.5,10);(57.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(59.42,13.07)"
%	 p2= "(58.18,13.07)"
%	 p1= "(58.18,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(62.62,13.07)"
%	 p2= "(61.38,13.07)"
%	 p1= "(61.38,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%</g>
%<circle p3= "(43.57,13.07)"
%	 p2= "(42.33,13.07)"
%	 p1= "(42.33,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(46.77,13.07)"
%	 p2= "(45.53,13.07)"
%	 p1= "(45.53,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-color= "#808080"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(49.97,13.07)"
%	 p2= "(48.73,13.07)"
%	 p1= "(48.73,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(53.17,13.07)"
%	 p2= "(51.93,13.07)"
%	 p1= "(51.93,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(56.37,13.07)"
%	 p2= "(55.13,13.07)"
%	 p1= "(55.13,11.83)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,15);(47.5,15);(47.5,10);(47.5,10)"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.25,15);(41.25,15);(41.25,10);(41.25,10)"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.88,15);(21.88,15);(21.88,10);(21.88,10)"
%	 stroke-width= "0.05"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.62,15);(15.62,15);(15.62,10);(15.62,10)"
%	 stroke-width= "0.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60.62,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_3$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_2^0$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_1^1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60.62,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A_2$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(19.08,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$C_1^2$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(108.75,25)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](57.5,10)
(63.75,10)
(63.75,5)
(0,5)(57.5,10)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](15.62,20)
(21.88,20)
(21.88,15)
(0,15)(15.62,20)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](47.5,20)
(47.5,15)
(0,15)
(41.25,20)(47.5,20)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](57.5,20)
(57.5,15)
(0,15)
(51.25,20)(57.5,20)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](57.5,5)
(63.75,5)
(63.75,0)
(57.5,0)(57.5,5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,5)
(57.5,5)
(57.5,0)
(0,0)(0,5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](63.75,5)
(108.75,5)
(108.75,0)
(63.75,0)(63.75,5)
\rput{90}(1.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(23.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(26.95,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](67.5,15)
(108.75,15)
(108.75,10)
(67.5,10)(67.5,15)
\rput{0}(68.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(72.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(75.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(78.45,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(81.65,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(84.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(88.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(91.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(94.45,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(97.65,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100.85,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(104.05,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(107.25,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(58.87,2.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(62.07,2.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(65.27,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(68.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(71.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(74.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(78.07,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(81.27,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(84.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(87.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(90.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(94.07,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(97.27,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(103.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(106.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(42.87,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(46.07,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(49.27,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(52.47,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.67,2.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\psline[linewidth=0.05,linecolor=gray](47.5,20)(47.5,15)
\psline[linewidth=0.05,linecolor=gray](21.88,20)(21.88,15)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](41.25,25)
(47.5,25)
(47.5,20)
(41.25,20)(41.25,25)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](15.62,25)
(21.88,25)
(21.88,20)
(15.62,20)(15.62,25)
\rput{0}(17.35,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,25)
(15.62,25)
(15.62,20)
(0,20)(0,25)
\rput{0}(1.35,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](25.62,25)
(41.25,25)
(41.25,20)
(25.62,20)(25.62,25)
\rput{0}(26.95,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,22.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(42.95,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(46.15,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(49.35,22.45){\psellipse[linewidth=0.15,linecolor=white,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](51.25,25)
(57.5,25)
(57.5,20)
(51.25,20)(51.25,25)
\rput{0}(52.55,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.75,22.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(54.38,22.5){$C_2^0$}
\rput(44.7,22.5){$C_2^1$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(57.5,15)
(57.5,10)
(0,10)(0,15)
\rput{0}(17.35,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(20.55,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(23.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(26.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(1.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(4.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(7.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(26.95,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(30.15,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(33.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(36.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](57.5,15)
(63.75,15)
(63.75,10)
(57.5,10)(57.5,15)
\rput{0}(58.8,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(62,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(42.95,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(46.15,12.45){\psellipse[linewidth=0.15,linecolor=gray,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(49.35,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(52.55,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.75,12.45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\psline[linewidth=0.05](47.5,15)(47.5,10)
\psline[linewidth=0.05](41.25,15)(41.25,10)
\psline[linewidth=0.05](21.88,15)(21.88,10)
\psline[linewidth=0.05](15.62,15)(15.62,10)
\rput(60.62,12.5){$B_3$}
\rput(44.38,12.5){$B_2^0$}
\rput(18.75,12.5){$B_1^1$}
\rput(60.62,2.5){$A_2$}
\rput(19.08,22.5){$C_1^2$}
\end{pspicture}


==> pictures/fig-natural-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 05 10:31:37 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="-5.14" y-max="43.12" auto-bounding="true">
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "solid"
%	 stroke-style= "dashed"
%	 points= "(0,2);(0,2);(15,26);(15,26);(15,26);(40,2);
%	(40,2)"
%	 stroke-width= "0.1"
%	 fill-color= "#cccccc"
%	 />
%<multicurve stroke-dasharray= "1.5;1.5"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(24.38,11.88);(24.38,11.88);(25.62,43.12);(25.62,43.12)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,26.25);(15,26.25);(23.75,12.5);(23.75,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(23.75,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$q$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.75,6.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$r$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,27.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$p$
%</text>
%<multicurve fill-style= "none"
%	 points= "(14.38,9.38);(14.38,9.38);(25,29.38);(25,29.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.12,29.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$u$
%</text>
%<multicurve stroke-dasharray= "1.5;1.5"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(14.38,8.75);(14.38,8.75);(15.62,42.5);(15.62,42.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(24.99,12.5)"
%	 p2= "(23.75,12.5)"
%	 p1= "(23.75,11.25)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(14.74,9.37)"
%	 p2= "(13.5,9.37)"
%	 p1= "(13.5,8.13)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(15.62,26.87)"
%	 p2= "(14.38,26.87)"
%	 p1= "(14.38,25.63)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.75,38.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A^{(k)}(r)$
%</text>
%<circle p3= "(25.62,29.74)"
%	 p2= "(24.38,29.74)"
%	 p1= "(24.38,28.5)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,38.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A^{(k)}(q)$
%</text>
%<pscurve stroke-dasharray= "1;1"
%	 fill-style= "solid"
%	 stroke-style= "dashed"
%	 closed= "false"
%	 curvature= "1;0.1;0"
%	 points= "(0,2);(0,2);(40,2);(41,4)"
%	 stroke-width= "0.1"
%	 fill-color= "#cccccc"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(40,43.12)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[linewidth=0.1,linestyle=dashed,dash=1 1,fillcolor=userFillColour,fillstyle=solid](0,2)
(15,26)(40,2)
\psline[linewidth=0.2,linestyle=dashed,dash=1.5 1.5](24.38,11.88)(25.62,43.12)
\psline(15,26.25)(23.75,12.5)
\rput(23.75,9.38){$q$}
\rput(13.75,6.25){$r$}
\rput(17.5,27.5){$p$}
\psline(14.38,9.38)(25,29.38)
\rput(28.12,29.38){$u$}
\psline[linewidth=0.2,linestyle=dashed,dash=1.5 1.5](14.38,8.75)(15.62,42.5)
\rput{0}(24.37,11.87){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(14.12,8.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(15,26.25){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(8.75,38.75){$A^{(k)}(r)$}
\rput{0}(25,29.12){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(32.5,38.75){$A^{(k)}(q)$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psecurve[linewidth=0.1,linestyle=dashed,dash=1 1,fillcolor=userFillColour,fillstyle=solid,curvature=1.0 0.1 0.0](0,2)(0,2)(40,2)(41,4)
\end{pspicture}


==> pictures/fig-property-l-3_2_1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Mar 11 23:41:45 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="96.87" y-min="0" y-max="23.38" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 points= "(7.5,15);(7.5,15);(80.62,22.5);(80.62,22.5);(80.62,22.5);(80.62,15);
%	(80.62,15);(80.62,15);(7.5,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.05"
%	 fill-color= "#cccccc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(8.12,15);(8.12,15);(56.88,21.88);(56.88,21.88);(56.88,21.88);(56.88,15);
%	(56.88,15);(56.88,15);(8.12,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.05"
%	 fill-color= "#cccccc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(1.25,5);(1.25,5);(96.87,5);(96.87,5);(96.87,5);(96.87,0);
%	(96.87,0);(96.87,0);(1.25,0);(1.25,0);(1.25,0);(1.25,5)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.75,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(53.75,15);(53.75,15);(65,15);(65,15);(65,15);(65,10);
%	(65,10);(65,10);(53.75,10);(53.75,10);(53.75,10);(53.75,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(80.62,22.5);(80.62,22.5);(62.5,12.5);(62.5,12.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(42.5,15);(42.5,15);(53.75,15);(53.75,15);(53.75,15);(53.75,10);
%	(53.75,10);(53.75,10);(42.5,10);(42.5,10);(42.5,10);(42.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(56.88,22.5);(56.88,22.5);(45.62,12.5);(45.62,12.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(63.12,13.12)"
%	 p2= "(61.88,13.12)"
%	 p1= "(61.88,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(59.38,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_s$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_r$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(71.25,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(77.5,15);(77.5,15);(88.75,15);(88.75,15);(88.75,15);(88.75,10);
%	(88.75,10);(88.75,10);(77.5,10);(77.5,10);(77.5,10);(77.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(81.24,23.12)"
%	 p2= "(80,23.12)"
%	 p1= "(80,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(83.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$B_t$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(93.12,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\dots$
%</text>
%<multicurve fill-style= "none"
%	 points= "(56.88,22.5);(56.88,22.5);(56.88,15);(56.88,15)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 />
%<circle p3= "(57.49,23.12)"
%	 p2= "(56.25,23.12)"
%	 p1= "(56.25,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(83.12,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$p$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(8.12,15);(8.12,15);(45.62,21.88);(45.62,21.88);(45.62,21.88);(45.62,15);
%	(45.62,15);(45.62,15);(8.12,15)"
%	 stroke-color= "#666666"
%	 stroke-width= "0.05"
%	 fill-color= "#999999"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\dots$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(8,15);(8,15);(22,22);(22,22);(22,22);(22,15);
%	(22,15);(22,15);(8,15)"
%	 stroke-color= "#333333"
%	 stroke-width= "0.05"
%	 fill-color= "#666666"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(18.75,15);(18.75,15);(30,15);(30,15);(30,15);(30,10);
%	(30,10);(30,10);(18.75,10);(18.75,10);(18.75,10);(18.75,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(33.12,22.5);(33.12,22.5);(21.88,12.5);(21.88,12.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(7.5,15);(7.5,15);(18.75,15);(18.75,15);(18.75,15);(18.75,10);
%	(18.75,10);(18.75,10);(7.5,10);(7.5,10);(7.5,10);(7.5,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(45.62,22.5);(45.62,22.5);(34.38,12.5);(34.38,12.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(46.24,23.12)"
%	 p2= "(45,23.12)"
%	 p1= "(45,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40.62,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$k_{s-1}$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.88,22.5);(21.88,22.5);(21.88,12.5);(21.88,12.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(21.88,22.5);(21.88,22.5);(10.62,12.5);(10.62,12.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(22.49,23.12)"
%	 p2= "(21.25,23.12)"
%	 p1= "(21.25,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(46.25,13.12)"
%	 p2= "(45.01,13.12)"
%	 p1= "(45.01,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50.62,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_{s-1}$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$k_r$
%</text>
%<circle p3= "(11.25,13.12)"
%	 p2= "(10.01,13.12)"
%	 p1= "(10.01,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(22.49,13.12)"
%	 p2= "(21.25,13.12)"
%	 p1= "(21.25,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.62,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_{r-1}$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$k_s$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(33.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45.62,22.5);(45.62,22.5);(45.62,12.5);(45.62,12.5)"
%	 stroke-width= "0.2"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(96.87,23.38)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\pspolygon[linewidth=0.05,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](7.5,15)
(80.62,22.5)
(80.62,15)(7.5,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\pspolygon[linewidth=0.05,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](8.12,15)
(56.88,21.88)
(56.88,15)(8.12,15)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](1.25,5)
(96.87,5)
(96.87,0)
(1.25,0)(1.25,5)
\rput(48.75,2.5){$A$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](53.75,15)
(65,15)
(65,10)
(53.75,10)(53.75,15)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](80.62,22.5)(62.5,12.5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](42.5,15)
(53.75,15)
(53.75,10)
(42.5,10)(42.5,15)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](56.88,22.5)(45.62,12.5)
\rput{0}(62.5,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(59.38,12.5){$b_s$}
\rput(26.25,12.5){$b_r$}
\rput(71.25,12.5){$\ldots$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](77.5,15)
(88.75,15)
(88.75,10)
(77.5,10)(77.5,15)
\rput{0}(80.62,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(83.75,12.5){$B_t$}
\rput(93.12,12.5){$\dots$}
\psline[linewidth=0.05,linecolor=gray](56.88,22.5)(56.88,15)
\rput{0}(56.87,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(83.12,22.5){$p$}
\newrgbcolor{userLineColour}{0.4 0.4 0.4}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linewidth=0.05,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](8.12,15)
(45.62,21.88)
(45.62,15)(8.12,15)
\rput(3.75,12.5){$\dots$}
\newrgbcolor{userLineColour}{0.2 0.2 0.2}
\newrgbcolor{userFillColour}{0.4 0.4 0.4}
\pspolygon[linewidth=0.05,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](8,15)
(22,22)
(22,15)(8,15)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](18.75,15)
(30,15)
(30,10)
(18.75,10)(18.75,15)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](33.12,22.5)(21.88,12.5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](7.5,15)
(18.75,15)
(18.75,10)
(7.5,10)(7.5,15)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](45.62,22.5)(34.38,12.5)
\rput{0}(45.62,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(40.62,22.5){$k_{s-1}$}
\psline[linewidth=0.2](21.88,22.5)(21.88,12.5)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](21.88,22.5)(10.62,12.5)
\rput{0}(21.87,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(45.63,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(50.62,12.5){$b_{s-1}$}
\rput(25,22.5){$k_r$}
\rput{0}(10.63,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(21.87,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(15.62,12.5){$b_{r-1}$}
\rput(60,22.5){$k_s$}
\rput(33.75,12.5){$\ldots$}
\psline[linewidth=0.2](45.62,22.5)(45.62,12.5)
\end{pspicture}


==> pictures/fig-property-l-3_2_2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Mar 18 00:04:32 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="11" x-max="88.75" y-min="0" y-max="23.38" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 points= "(73,22);(73,22);(73,15.12);(73,15.12);(73,15.12);(11,15.12);
%	(11,15.12);(11,15.12);(72.62,22.12);(72.62,22.12);(72.62,22.12);(73,22)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#cccccc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(49.38,21.88);(49.38,21.88);(49.38,15);(49.38,15);(49.38,15);(11.38,14.88);
%	(11.38,14.88);(11.38,14.88);(49,22);(49,22);(49,22);(49.38,21.88)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#cccccc"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(38,22);(38,22);(38,15.12);(38,15.12);(38,15.12);(11,15.12);
%	(11,15.12);(11,15.12);(37.62,22.12);(37.62,22.12);(37.62,22.12);(38,22)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#999999"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(14.38,21.88);(14.38,21.88);(14.38,15);(14.38,15);(14.38,15);(11,15);
%	(11,15);(11,15);(14,22);(14,22);(14,22);(14.38,21.88)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 fill-color= "#666666"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(11.25,5);(11.25,5);(88.75,5);(88.75,5);(88.75,5);(88.75,0);
%	(88.75,0);(88.75,0);(11.25,0);(11.25,0);(11.25,0);(11.25,5)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(41.25,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(46.25,15);(46.25,15);(57.5,15);(57.5,15);(57.5,15);(57.5,10);
%	(57.5,10);(57.5,10);(46.25,10);(46.25,10);(46.25,10);(46.25,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(73.12,22.5);(73.12,22.5);(55,12.5);(55,12.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(35,15);(35,15);(46.25,15);(46.25,15);(46.25,15);(46.25,10);
%	(46.25,10);(46.25,10);(35,10);(35,10);(35,10);(35,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(49.38,22.5);(49.38,22.5);(38.12,12.5);(38.12,12.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(55.62,13.12)"
%	 p2= "(54.38,13.12)"
%	 p1= "(54.38,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.88,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_s$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_r$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(63.75,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(70,15);(70,15);(81.25,15);(81.25,15);(81.25,15);(81.25,10);
%	(81.25,10);(81.25,10);(70,10);(70,10);(70,10);(70,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<circle p3= "(73.74,23.12)"
%	 p2= "(72.5,23.12)"
%	 p1= "(72.5,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(76.25,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$B_t$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85.62,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\dots$
%</text>
%<multicurve fill-style= "none"
%	 points= "(49.38,22.5);(49.38,22.5);(49.38,15);(49.38,15)"
%	 stroke-color= "#808080"
%	 stroke-width= "0.05"
%	 />
%<circle p3= "(49.99,23.12)"
%	 p2= "(48.75,23.12)"
%	 p1= "(48.75,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75.62,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$p$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(11.25,15);(11.25,15);(22.5,15);(22.5,15);(22.5,15);(22.5,10);
%	(22.5,10);(22.5,10);(11.25,10);(11.25,10);(11.25,10);(11.25,15)"
%	 stroke-width= "0.05"
%	 fill-color= "#f0f0f0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(25.62,22.5);(25.62,22.5);(14.38,12.5);(14.38,12.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(38.12,22.5);(38.12,22.5);(38.12,12.5);(38.12,12.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(38.12,22.5);(38.12,22.5);(26.88,12.5);(26.88,12.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(38.74,23.12)"
%	 p2= "(37.5,23.12)"
%	 p1= "(37.5,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(33.12,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$k_{s-1}$
%</text>
%<multicurve fill-style= "none"
%	 points= "(14.38,22.5);(14.38,22.5);(14.38,12.5);(14.38,12.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(38.75,13.12)"
%	 p2= "(37.51,13.12)"
%	 p1= "(37.51,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(43.12,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_{s-1}$
%</text>
%<circle p3= "(14.99,13.12)"
%	 p2= "(13.75,13.12)"
%	 p1= "(13.75,11.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$k_s$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ldots$
%</text>
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(14.38,22.5);(14.38,22.5);(64.38,2.5);(64.38,2.5)"
%	 stroke-width= "0.2"
%	 />
%<circle p3= "(64.62,3.12)"
%	 p2= "(63.38,3.12)"
%	 p1= "(63.38,1.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(67.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_0$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$b_1$
%</text>
%<circle p3= "(14.99,23.12)"
%	 p2= "(13.75,23.12)"
%	 p1= "(13.75,21.88)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$k_1$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(88.75,23.38)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](73,22)
(73,15.12)
(11,15.12)
(72.62,22.12)(73,22)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](49.38,21.88)
(49.38,15)
(11.38,14.88)
(49,22)(49.38,21.88)
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](38,22)
(38,15.12)
(11,15.12)
(37.62,22.12)(38,22)
\newrgbcolor{userFillColour}{0.4 0.4 0.4}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](14.38,21.88)
(14.38,15)
(11,15)
(14,22)(14.38,21.88)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](11.25,5)
(88.75,5)
(88.75,0)
(11.25,0)(11.25,5)
\rput(41.25,2.5){$A$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](46.25,15)
(57.5,15)
(57.5,10)
(46.25,10)(46.25,15)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](73.12,22.5)(55,12.5)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](35,15)
(46.25,15)
(46.25,10)
(35,10)(35,15)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](49.38,22.5)(38.12,12.5)
\rput{0}(55,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(51.88,12.5){$b_s$}
\rput(18.75,12.5){$b_r$}
\rput(63.75,12.5){$\ldots$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](70,15)
(81.25,15)
(81.25,10)
(70,10)(70,15)
\rput{0}(73.12,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(76.25,12.5){$B_t$}
\rput(85.62,12.5){$\dots$}
\psline[linewidth=0.05,linecolor=gray](49.38,22.5)(49.38,15)
\rput{0}(49.37,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(75.62,22.5){$p$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](11.25,15)
(22.5,15)
(22.5,10)
(11.25,10)(11.25,15)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](25.62,22.5)(14.38,12.5)
\psline[linewidth=0.2](38.12,22.5)(38.12,12.5)
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](38.12,22.5)(26.88,12.5)
\rput{0}(38.12,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(33.12,22.5){$k_{s-1}$}
\psline[linewidth=0.2](14.38,22.5)(14.38,12.5)
\rput{0}(38.13,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(43.12,12.5){$b_{s-1}$}
\rput{0}(14.37,12.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(52.5,22.5){$k_s$}
\rput(26.25,12.5){$\ldots$}
\psline[linewidth=0.2,linestyle=dashed,dash=1 1](14.38,22.5)(64.38,2.5)
\rput{0}(64,2.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(67.5,2.5){$b_0$}
\rput(17.5,12.5){$b_1$}
\rput{0}(14.37,22.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(17.5,22.5){$k_1$}
\end{pspicture}


==> pictures/fig-pulling.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Feb 09 18:29:41 CET 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="87.5" y-min="0" y-max="25" auto-bounding="true">
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(15,10);(15,10);(15,5);(15,5);(15,5);(-0,5);
%	(-0,5);(-0,5);(0,10);(0,10);(0,10);(15,10)"
%	 fill-color= "#a0a0a0"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(30,10);(30,10);(30,5);(30,5);(30,5);(0,5);
%	(0,5);(0,5);(15,10);(15,10);(15,10);(30,10)"
%	 fill-color= "#b4b4b4"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(57.5,10);(57.5,10);(57.5,5);(57.5,5);(57.5,5);(0,5);
%	(0,5);(0,5);(42.5,10);(42.5,10);(42.5,10);(57.5,10)"
%	 fill-color= "#c8c8c8"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(72.5,10);(72.5,10);(72.5,5);(72.5,5);(72.5,5);(0,5);
%	(0,5);(0,5);(57.5,10);(57.5,10);(57.5,10);(72.5,10)"
%	 fill-color= "#dcdcdc"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(15,20);(15,20);(15,15);(15,15);(15,15);(0,15);
%	(0,15);(0,15);(6.25,20);(6.25,20);(6.25,20);(15,20)"
%	 fill-color= "#a0a0a0"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(30,20);(30,20);(30,15);(30,15);(30,15);(0,15);
%	(0,15);(0,15);(21.25,20);(21.25,20);(21.25,20);(30,20)"
%	 fill-color= "#b4b4b4"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 stroke-color= "#808080"
%	 points= "(57.5,20);(57.5,20);(57.5,15);(57.5,15);(57.5,15);(0,15);
%	(0,15);(0,15);(48.75,20);(48.75,20);(48.75,20);(57.5,20)"
%	 fill-color= "#c8c8c8"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.05"
%	 points= "(-0,5);(-0,5);(87.5,5);(87.5,5);(87.5,5);(87.5,0);
%	(87.5,0);(87.5,0);(-0,0);(-0,0);(-0,0);(-0,5)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$A$
%</text>
%<g>
%<multicurve stroke-width= "0.05"
%	 points= "(0,15);(0,15);(15,15);(15,15);(15,15);(15,10);
%	(15,10);(15,10);(0,10);(0,10);(0,10);(0,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_1$
%</text>
%</g>
%<text text-vert-align= "center-v"
%	 anchor-point= "(36.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\ldots$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(15,15);(15,15);(30,15);(30,15);(30,15);(30,10);
%	(30,10);(30,10);(15,10);(15,10);(15,10);(15,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_2$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(21.25,25);(21.25,25);(30,25);(30,25);(30,25);(30,20);
%	(30,20);(30,20);(21.25,20);(21.25,20);(21.25,20);(21.25,25)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$W_2$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(48.75,25);(48.75,25);(57.5,25);(57.5,25);(57.5,25);(57.5,20);
%	(57.5,20);(57.5,20);(48.75,20);(48.75,20);(48.75,20);(48.75,25)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(53.75,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$W_k$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(6.25,25);(6.25,25);(15,25);(15,25);(15,25);(15,20);
%	(15,20);(15,20);(6.25,20);(6.25,20);(6.25,20);(6.25,25)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(11.25,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$W_1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(36.25,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\ldots$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(57.5,15);(57.5,15);(72.5,15);(72.5,15);(72.5,15);(72.5,10);
%	(72.5,10);(72.5,10);(57.5,10);(57.5,10);(57.5,10);(57.5,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_{k+1}$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(42.5,15);(42.5,15);(57.5,15);(57.5,15);(57.5,15);(57.5,10);
%	(57.5,10);(57.5,10);(42.5,10);(42.5,10);(42.5,10);(42.5,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_k$
%</text>
%<multicurve stroke-width= "0.05"
%	 points= "(72.5,15);(72.5,15);(87.5,15);(87.5,15);(87.5,15);(87.5,10);
%	(87.5,10);(87.5,10);(72.5,10);(72.5,10);(72.5,10);(72.5,15)"
%	 fill-color= "#f0f0f0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$B_0$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\ldots$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\ldots$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(87.5,25)
\newrgbcolor{userFillColour}{0.63 0.63 0.63}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](15,10)
(15,5)
(-0,5)
(0,10)(15,10)
\newrgbcolor{userFillColour}{0.71 0.71 0.71}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](30,10)
(30,5)
(0,5)
(15,10)(30,10)
\newrgbcolor{userFillColour}{0.78 0.78 0.78}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](57.5,10)
(57.5,5)
(0,5)
(42.5,10)(57.5,10)
\newrgbcolor{userFillColour}{0.86 0.86 0.86}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](72.5,10)
(72.5,5)
(0,5)
(57.5,10)(72.5,10)
\newrgbcolor{userFillColour}{0.63 0.63 0.63}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](15,20)
(15,15)
(0,15)
(6.25,20)(15,20)
\newrgbcolor{userFillColour}{0.71 0.71 0.71}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](30,20)
(30,15)
(0,15)
(21.25,20)(30,20)
\newrgbcolor{userFillColour}{0.78 0.78 0.78}
\pspolygon[linewidth=0.05,linecolor=gray,fillcolor=userFillColour,fillstyle=solid](57.5,20)
(57.5,15)
(0,15)
(48.75,20)(57.5,20)
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](-0,5)
(87.5,5)
(87.5,0)
(-0,0)(-0,5)
\rput(45,2.5){$A$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](0,15)
(15,15)
(15,10)
(0,10)(0,15)
\rput(7.5,12.5){$B_1$}
\rput(36.25,12.5){$\ldots$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](15,15)
(30,15)
(30,10)
(15,10)(15,15)
\rput(22.5,12.5){$B_2$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](21.25,25)
(30,25)
(30,20)
(21.25,20)(21.25,25)
\rput(26.25,22.5){$W_2$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](48.75,25)
(57.5,25)
(57.5,20)
(48.75,20)(48.75,25)
\rput(53.75,22.5){$W_k$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](6.25,25)
(15,25)
(15,20)
(6.25,20)(6.25,25)
\rput(11.25,22.5){$W_1$}
\rput(36.25,22.5){$\ldots$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](57.5,15)
(72.5,15)
(72.5,10)
(57.5,10)(57.5,15)
\rput(65,12.5){$B_{k+1}$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](42.5,15)
(57.5,15)
(57.5,10)
(42.5,10)(42.5,15)
\rput(50,12.5){$B_k$}
\newrgbcolor{userFillColour}{0.94 0.94 0.94}
\pspolygon[linewidth=0.05,fillcolor=userFillColour,fillstyle=solid](72.5,15)
(87.5,15)
(87.5,10)
(72.5,10)(72.5,15)
\rput(80,12.5){$B_0$}
\rput(2.5,22.5){$\ldots$}
\rput(17.5,22.5){$\ldots$}
\end{pspicture}


==> pictures/pic-2dim.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sun Feb 11 15:09:22 CET 2007
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="59.38" y-min="0" y-max="52.5" auto-bounding="true">
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(44.38,38.12)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$y_{i+1}$
%</text>
%<multicurve points="(25,30.62);(25,30.62);(25,51.89);(25,51.89)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<multicurve points="(53.12,30);(53.12,30);(26.24,30);(26.24,30)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<multicurve points="(0,0);(0,0);(57.5,0);(57.5,0)"
%	 stroke-width="0.35"
%	 fill-color="#ffffff" fill-style="solid"
%	 right-arrow="head" arrow-head-width-minimum="0.6" arrow-head-length-scale="2.3" arrow-head-inset-scale="0" arrow-tbar-width-minimum="0" arrow-bracket-length-scale="0" arrow-rbracket-length-scale="0" />
%<multicurve points="(0,0);(0,0);(0,52.5);(0,52.5)"
%	 stroke-width="0.35"
%	 fill-color="#ffffff" fill-style="solid"
%	 right-arrow="head" arrow-head-width-minimum="0.6" arrow-head-length-scale="2.3" arrow-head-inset-scale="0" arrow-tbar-width-minimum="0" arrow-bracket-length-scale="0" arrow-rbracket-length-scale="0" />
%<multicurve points="(53.12,45);(53.12,45);(10,45);(10,45)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(7.5,42.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_{i-1}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(35,42.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$y_i$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(22.5,27.5)" text-frame="noframe"
%	
%	 fill-color="#ffffff" fill-style="solid"
%	 >
%$x_{i+1}$
%</text>
%<g>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(31.24,23.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(32.5,22.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%</g>
%<g>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(5,50)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(6.24,48.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(7.5,47.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%</g>
%<g>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(49.39,5.62)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(50.62,4.38)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(51.89,3.12)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%</g>
%<g>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(41.25,36.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(42.5,35)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(43.75,33.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%.
%</text>
%</g>
%<circle p1="(24.37,29.38)" p2="(24.37,30.62)" p3="(25.62,30.62)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<circle p1="(9.37,44.38)" p2="(9.37,45.62)" p3="(10.62,45.62)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(50,31.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$y_j$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(59.38,2.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$L_1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(2.5,52.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$L_2$
%</text>
%<multicurve points="(37.5,18.12);(37.5,18.12);(37.5,51.88);(37.5,51.88)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(34.37,15.62)" text-frame="noframe"
%	
%	 fill-color="#ffffff" fill-style="solid"
%	 >
%$x_j$
%</text>
%<g>
%<multicurve points="(53.12,17.5);(53.12,17.5);(38.12,17.5);(38.12,17.5)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<circle p1="(36.87,16.88)" p2="(36.87,18.12)" p3="(38.12,18.12)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%</g>
%<multicurve points="(15.01,41.25);(15.01,41.25);(15,51.88);(15,51.88)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(12.51,37.5)" text-frame="noframe"
%	
%	 fill-color="#ffffff" fill-style="solid"
%	 >
%$x_{i}$
%</text>
%<multicurve points="(53.12,40);(53.12,40);(15.63,40);(15.63,40)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<circle p1="(14.38,39.38)" p2="(14.38,40.62)" p3="(15.63,40.62)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<circle p1="(36.88,39.38)" p2="(36.88,40.62)" p3="(38.13,40.62)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<circle p1="(38.88,37.38)" p2="(38.88,38.62)" p3="(40.13,38.62)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<circle p1="(44.88,31.38)" p2="(44.88,32.62)" p3="(46.13,32.62)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<multicurve points="(47.5,8.12);(47.5,8.12);(47.5,51.88);(47.5,51.88)"
%	 stroke-width="0.15" stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(42.5,4.38)" text-frame="noframe"
%	
%	 fill-color="#ffffff" fill-style="solid"
%	 >
%$x_{j+1}$
%</text>
%<circle p1="(46.87,6.88)" p2="(46.87,8.12)" p3="(48.12,8.12)" closure="plain"
%	 stroke-width="0.15"
%	 fill-color="#ffffff" fill-style="solid"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(59.38,52.5)
\rput(44.38,38.12){$y_{i+1}$}
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](25,30.62)(25,51.89)
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](53.12,30)(26.24,30)
\psline[linewidth=0.35,fillcolor=white,fillstyle=solid,arrowsize=0.6 2,arrowlength=2.3,arrowinset=0,tbarsize=0 5,bracketlength=0,rbracketlength=0]{->}(0,0)(57.5,0)
\psline[linewidth=0.35,fillcolor=white,fillstyle=solid,arrowsize=0.6 2,arrowlength=2.3,arrowinset=0,tbarsize=0 5,bracketlength=0,rbracketlength=0]{->}(0,0)(0,52.5)
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](53.12,45)(10,45)
\rput(7.5,42.5){$x_{i-1}$}
\rput(35,42.5){$y_i$}
\rput(22.5,27.5){$x_{i+1}$}
\rput(30,25){.}
\rput(31.24,23.75){.}
\rput(32.5,22.5){.}
\rput(5,50){.}
\rput(6.24,48.75){.}
\rput(7.5,47.5){.}
\rput(49.39,5.62){.}
\rput(50.62,4.38){.}
\rput(51.89,3.12){.}
\rput(41.25,36.25){.}
\rput(42.5,35){.}
\rput(43.75,33.75){.}
\rput{0}(25,30){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(9.99,45){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(50,31.25){$y_j$}
\rput(59.38,2.5){$L_1$}
\rput(2.5,52.5){$L_2$}
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](37.5,18.12)(37.5,51.88)
\rput(34.37,15.62){$x_j$}
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](53.12,17.5)(38.12,17.5)
\rput{0}(37.5,17.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](15.01,41.25)(15,51.88)
\rput(12.51,37.5){$x_{i}$}
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](53.12,40)(15.63,40)
\rput{0}(15,40){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(37.5,40){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(39.5,38){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(45.5,32){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\psline[linewidth=0.15,linestyle=dashed,dash=1 1,fillcolor=white,fillstyle=solid](47.5,8.12)(47.5,51.88)
\rput(42.5,4.38){$x_{j+1}$}
\rput{0}(47.5,7.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\end{pspicture}


==> pictures/pic-fact1_4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 08 20:26:06 CET 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="90" y-min="0.62" y-max="25.62" auto-bounding="true">
%<g>
%<multicurve fill-style= "solid"
%	 stroke-width= "0.1"
%	 points= "(50,13.12);(50,13.12);(30,13.12);(30,13.12);(30,13.12);(10,3.12);
%	(10,3.12);(10,3.12);(50,3.12);(50,3.12);(50,3.12);(50,13.12)"
%	 fill-color= "#c0c0c0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.2"
%	 points= "(5,3.12);(5,3.12);(90,3.12);(90,3.12)"
%	 />
%<multicurve fill-style= "solid"
%	 stroke-width= "0.1"
%	 points= "(85,13.12);(85,13.12);(65,13.12);(65,13.12);(65,13.12);(10,3.12);
%	(10,3.12);(10,3.12);(85,3.12);(85,3.12);(85,3.12);(85,13.12)"
%	 fill-color= "#c0c0c0"
%	 />
%<ellipse p3= "(50,11.88)"
%	 p2= "(50,14.38)"
%	 p1= "(30,14.38)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#ffffff"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(85,11.88)"
%	 p2= "(85,14.38)"
%	 p1= "(65,14.38)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#ffffff"
%	 angle-start= "0"
%	 />
%<multicurve stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(50,13.12);(50,13.12);(50,3.12);(50,3.12)"
%	 stroke-style= "dashed"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,3.12);(70,3.12);(70,13.12);(70,13.12)"
%	 />
%<circle p3= "(70.62,3.74)"
%	 p2= "(69.38,3.74)"
%	 p1= "(69.38,2.5)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(76.25,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_j$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,13.12);(70,13.12);(70,23.12);(70,23.12)"
%	 />
%<circle p3= "(70.62,23.74)"
%	 p2= "(69.38,23.74)"
%	 p1= "(69.38,22.5)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(45.62,13.74)"
%	 p2= "(44.38,13.74)"
%	 p1= "(44.38,12.5)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<circle p3= "(70.62,13.74)"
%	 p2= "(69.38,13.74)"
%	 p1= "(69.38,12.5)"
%	 closure= "plain"
%	 fill-style= "solid"
%	 stroke-width= "0.15"
%	 fill-color= "#ffffff"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(57.5,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$B_i$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,25.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$c$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,16.24)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$b$
%</text>
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 points= "(50,13.12);(50,13.12);(65,13.12);(65,13.12)"
%	 stroke-style= "dotted"
%	 />
%</g>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(90,25.62)
\pspolygon[linewidth=0.1,fillcolor=lightgray,fillstyle=solid](50,13.12)
(30,13.12)
(10,3.12)
(50,3.12)(50,13.12)
\psline[linewidth=0.2](5,3.12)(90,3.12)
\pspolygon[linewidth=0.1,fillcolor=lightgray,fillstyle=solid](85,13.12)
(65,13.12)
(10,3.12)
(85,3.12)(85,13.12)
\rput{0}(40,13.12){\psellipse[fillcolor=white,fillstyle=solid](0,0)(10,-1.25)}
\rput{0}(75,13.12){\psellipse[fillcolor=white,fillstyle=solid](0,0)(10,-1.25)}
\psline[linewidth=0.1,linestyle=dashed,dash=1 1](50,13.12)(50,3.12)
\psline(70,3.12)(70,13.12)
\rput{0}(70,3.12){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(76.25,9.38){$B_j$}
\psline(70,13.12)(70,23.12)
\rput{0}(70,23.12){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(45,13.12){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(70,13.12){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput(57.5,0.62){$A$}
\rput(37.5,10){$B_i$}
\rput(70,25.62){$c$}
\rput(45,16.24){$b$}
\psline[linestyle=dotted,dotsep=2](50,13.12)(65,13.12)
\end{pspicture}


==> pictures/pic-low-b.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Oct 16 16:01:33 CEST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="110" y-min="0" y-max="136.25" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 right-arrow= "disk-centered"
%	 fill-color= "#c0c0c0"
%	 left-arrow= "disk-centered"
%	 stroke-style= "none"
%	 points= "(70,97.5);(70,97.5);(100,97.5);(100,97.5);(100,97.5);(100,87.5);
%	(100,87.5);(100,87.5);(10,87.5);(10,87.5);(10,87.5);(70,97.5)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#808080"
%	 stroke-style= "none"
%	 points= "(17.5,97.5);(17.5,97.5);(10,97.5);(10,97.5);(10,97.5);(17.5,107.5);
%	(17.5,107.5);(17.5,107.5);(17.5,107.5);(17.5,107.5);(17.5,107.5);(17.5,97.5)"
%	 />
%<multicurve stroke-color= "#808080"
%	 fill-style= "none"
%	 points= "(10,107.5);(10,107.5);(10,97.5);(10,97.5)"
%	 />
%<multicurve stroke-color= "#c0c0c0"
%	 fill-style= "none"
%	 points= "(10,72.5);(10,72.5);(10,62.5);(10,62.5)"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "disk-centered"
%	 fill-color= "#c0c0c0"
%	 left-arrow= "disk-centered"
%	 stroke-style= "none"
%	 points= "(10,62.5);(10,62.5);(17.5,62.5);(17.5,62.5);(17.5,62.5);(17.5,72.5);
%	(17.5,72.5);(17.5,72.5);(17.5,72.5);(17.5,72.5);(17.5,72.5);(10,62.5)"
%	 />
%<parallelogram p3= "(40,87.5)"
%	 fill-style= "solid"
%	 p1= "(10,97.5)"
%	 right-arrow= "disk-centered"
%	 fill-color= "#c0c0c0"
%	 left-arrow= "disk-centered"
%	 p2= "(40,97.5)"
%	 stroke-style= "none"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#808080"
%	 stroke-style= "none"
%	 points= "(55,87.5);(55,87.5);(10,87.5);(10,87.5);(10,87.5);(47.5,97.5);
%	(47.5,97.5);(47.5,97.5);(55,97.5);(55,97.5);(55,97.5);(55,87.5)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#808080"
%	 stroke-style= "none"
%	 points= "(40,97.5);(40,97.5);(10,97.5);(10,97.5);(10,97.5);(32.5,107.5);
%	(32.5,107.5);(32.5,107.5);(40,107.5);(40,107.5);(40,107.5);(40,97.5)"
%	 />
%<parallelogram p3= "(40,122.5)"
%	 fill-style= "solid"
%	 p1= "(10,132.5)"
%	 right-arrow= "disk-centered"
%	 fill-color= "#808080"
%	 left-arrow= "disk-centered"
%	 p2= "(40,132.5)"
%	 stroke-style= "none"
%	 />
%<multicurve fill-style= "solid"
%	 right-arrow= "disk-centered"
%	 fill-color= "#c0c0c0"
%	 left-arrow= "disk-centered"
%	 stroke-style= "none"
%	 points= "(70,132.5);(70,132.5);(100,132.5);(100,132.5);(100,132.5);(100,122.5);
%	(100,122.5);(100,122.5);(10,122.5);(10,122.5);(10,122.5);(70,132.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$2$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$3$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$4$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$5$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$6$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$7$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$8$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$9$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(77.5,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$10$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$11$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(92.5,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$12$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,120)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$13$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$14$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$15$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$16$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$17$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$18$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(104.38,122.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$A$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,132.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$B_1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(105,132.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$B_0$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(77.5,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$2$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$3$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(92.5,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$4$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,135.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$5$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$6$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$7$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$8$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,95)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$14$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,95)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$15$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,95)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$16$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,95)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$17$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,95)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$18$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,110.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$6$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,110.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$7$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,110.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$14$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,110.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$15$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,100)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$19$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,100)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$20$
%</text>
%<parallelogram p3= "(40,52.5)"
%	 fill-style= "solid"
%	 p1= "(10,62.5)"
%	 right-arrow= "disk-centered"
%	 fill-color= "#c0c0c0"
%	 left-arrow= "disk-centered"
%	 p2= "(40,62.5)"
%	 stroke-style= "none"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#c0c0c0"
%	 stroke-style= "none"
%	 points= "(55,52.5);(55,52.5);(10,52.5);(10,52.5);(10,52.5);(47.5,62.5);
%	(47.5,62.5);(47.5,62.5);(55,62.5);(55,62.5);(55,62.5);(55,52.5)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#c0c0c0"
%	 stroke-style= "none"
%	 points= "(40,62.5);(40,62.5);(10,62.5);(10,62.5);(10,62.5);(32.5,72.5);
%	(32.5,72.5);(32.5,72.5);(40,72.5);(40,72.5);(40,72.5);(40,62.5)"
%	 />
%<multicurve stroke-color= "#808080"
%	 fill-style= "solid"
%	 right-arrow= "disk-centered"
%	 fill-color= "#c0c0c0"
%	 left-arrow= "disk-centered"
%	 stroke-style= "none"
%	 stroke-width= "0.1"
%	 points= "(70,62.5);(70,62.5);(100,62.5);(100,62.5);(100,62.5);(100,52.5);
%	(100,52.5);(100,52.5);(10,52.5);(10,52.5);(10,52.5);(70,62.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,50)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$8$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,60)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$16$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,65.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 stroke-style= "none"
%	 >
%$21$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,75.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$16$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,75.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$19$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,75.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$8$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$9$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(77.5,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$10$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$11$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(92.5,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$12$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$13$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,50)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$9$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(77.5,50)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$10$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,50)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$11$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(92.5,50)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$12$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,50)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$13$
%</text>
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(100,20);(100,20);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(92.5,20);(92.5,20);(92.5,10);(92.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(85,20);(85,20);(85,10);(85,10)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(77.5,20);(77.5,20);(77.5,10);(77.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(70,20);(70,20);(70,10);(70,10)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(100,30.62);(100,30.62);(100,20.62);(100,20.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(92.5,30.62);(92.5,30.62);(92.5,20.62);(92.5,20.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(85,30.62);(85,30.62);(85,20.62);(85,20.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(77.5,30.62);(77.5,30.62);(77.5,20.62);(77.5,20.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(70,30.62);(70,30.62);(70,20.62);(70,20.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(40,10);(40,10);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(32.5,10);(32.5,10);(32.5,0);(32.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(25,10);(25,10);(25,0);(25,0)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(17.5,10);(17.5,10);(17.5,0);(17.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(10,10);(10,10);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(62.5,18.75);(62.5,18.75);(62.5,8.75);(62.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(47.5,15.62);(47.5,15.62);(47.5,5.62);(47.5,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(55,15.62);(55,15.62);(55,5.62);(55,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(62.5,29.38);(62.5,29.38);(62.5,19.38);(62.5,19.38)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(47.5,26.25);(47.5,26.25);(47.5,16.25);(47.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(55,27.5);(55,27.5);(55,17.5);(55,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(40,25);(40,25);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(32.5,25);(32.5,25);(32.5,15);(32.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(25,23.75);(25,23.75);(25,13.75);(25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(17.5,22.5);(17.5,22.5);(17.5,12.5);(17.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(10,20.62);(10,20.62);(10,10.62);(10,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,10)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$A$
%</text>
%<multicurve fill-style= "none"
%	 stroke-style= "dotted"
%	 stroke-width= "0.2"
%	 points= "(6.25,20.62);(6.25,20.62);(41.25,20.62);(41.25,20.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,21.25)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$B$
%</text>
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(47.5,36.88);(47.5,36.88);(47.5,26.88);(47.5,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(55,38.12);(55,38.12);(55,28.12);(55,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(32.5,35.62);(32.5,35.62);(32.5,25.62);(32.5,25.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(40,35.62);(40,35.62);(40,25.62);(40,25.62)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(25,34.38);(25,34.38);(25,24.38);(25,24.38)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(17.5,33.12);(17.5,33.12);(17.5,23.12);(17.5,23.12)"
%	 />
%<multicurve fill-style= "none"
%	 right-arrow= "t-bar-flushed"
%	 left-arrow= "t-bar-flushed"
%	 points= "(10,31.25);(10,31.25);(10,21.25);(10,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-style= "dotted"
%	 stroke-width= "0.2"
%	 points= "(6.25,31.25);(6.25,31.25);(105,31.25);(105,31.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,31.88)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$C$
%</text>
%<multicurve fill-style= "none"
%	 stroke-style= "dotted"
%	 stroke-width= "0.2"
%	 points= "(45.62,20.62);(45.62,20.62);(56.25,20.62);(56.25,20.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-style= "dotted"
%	 stroke-width= "0.2"
%	 points= "(70,20.62);(70,20.62);(105,20.62);(105,20.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.75,22.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$B_1$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.25,22.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$B_2$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.25,22.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$B_0$
%</text>
%<multicurve fill-style= "none"
%	 stroke-style= "dotted"
%	 stroke-width= "0.2"
%	 points= "(60,20.62);(60,20.62);(65.62,20.62);(65.62,20.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65.62,22.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$B_3$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(59.38,98.75)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$B_2$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65.62,65.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$B_3$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,60)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$17$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,60)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$18$
%</text>
%<multicurve fill-style= "solid"
%	 fill-color= "#949494"
%	 stroke-style= "none"
%	 points= "(25,62.5);(25,62.5);(10,62.5);(10,62.5);(10,62.5);(25,72.5);
%	(25,72.5);(25,72.5);(25,72.5);(25,72.5);(25,72.5);(25,62.5)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#949494"
%	 stroke-style= "none"
%	 points= "(47.5,62.5);(47.5,62.5);(10,62.5);(10,62.5);(10,62.5);(47.5,72.5);
%	(47.5,72.5);(47.5,72.5);(47.5,72.5);(47.5,72.5);(47.5,72.5);(47.5,62.5)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#808080"
%	 stroke-style= "none"
%	 points= "(55,62.5);(55,62.5);(10,62.5);(10,62.5);(10,62.5);(55,72.5);
%	(55,72.5);(55,72.5);(55,72.5);(55,72.5);(55,72.5);(55,62.5)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#808080"
%	 stroke-style= "none"
%	 points= "(62.5,52.5);(62.5,52.5);(10,52.5);(10,52.5);(10,52.5);(62.5,62.5);
%	(62.5,62.5);(62.5,62.5);(62.5,62.5);(62.5,62.5);(62.5,62.5);(62.5,52.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,60)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$20$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,60)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 right-arrow= "disk-centered"
%	 left-arrow= "disk-centered"
%	 >
%$19$
%</text>
%<g>
%<circle closure= "plain"
%	 p3= "(10.62,53.37)"
%	 fill-style= "solid"
%	 p1= "(9.38,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,53.37)"
%	 fill-style= "solid"
%	 p1= "(16.88,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(25.62,53.37)"
%	 fill-style= "solid"
%	 p1= "(24.38,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(24.38,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.12,53.37)"
%	 fill-style= "solid"
%	 p1= "(31.88,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.62,53.37)"
%	 fill-style= "solid"
%	 p1= "(39.38,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(48.12,53.37)"
%	 fill-style= "solid"
%	 p1= "(46.88,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(46.88,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(55.62,53.37)"
%	 fill-style= "solid"
%	 p1= "(54.38,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(54.38,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(63.12,53.37)"
%	 fill-style= "solid"
%	 p1= "(61.88,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(61.88,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(70.62,53.37)"
%	 fill-style= "solid"
%	 p1= "(69.38,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(69.38,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(78.12,53.37)"
%	 fill-style= "solid"
%	 p1= "(76.88,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(76.88,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(85.62,53.37)"
%	 fill-style= "solid"
%	 p1= "(84.38,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(84.38,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(93.12,53.37)"
%	 fill-style= "solid"
%	 p1= "(91.88,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(91.88,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(100.62,53.37)"
%	 fill-style= "solid"
%	 p1= "(99.38,52.13)"
%	 fill-color= "#ffffff"
%	 p2= "(99.38,53.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(10.62,63.37)"
%	 fill-style= "solid"
%	 p1= "(9.38,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,63.37)"
%	 fill-style= "solid"
%	 p1= "(16.88,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(25.62,63.37)"
%	 fill-style= "solid"
%	 p1= "(24.38,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(24.38,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.12,63.37)"
%	 fill-style= "solid"
%	 p1= "(31.88,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.62,63.37)"
%	 fill-style= "solid"
%	 p1= "(39.38,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(48.12,63.37)"
%	 fill-style= "solid"
%	 p1= "(46.88,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(46.88,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(55.62,63.37)"
%	 fill-style= "solid"
%	 p1= "(54.38,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(54.38,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(63.12,63.37)"
%	 fill-style= "solid"
%	 p1= "(61.88,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(61.88,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(70.62,63.37)"
%	 fill-style= "solid"
%	 p1= "(69.38,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(69.38,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(78.12,63.37)"
%	 fill-style= "solid"
%	 p1= "(76.88,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(76.88,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(85.62,63.37)"
%	 fill-style= "solid"
%	 p1= "(84.38,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(84.38,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(93.12,63.37)"
%	 fill-style= "solid"
%	 p1= "(91.88,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(91.88,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(100.62,63.37)"
%	 fill-style= "solid"
%	 p1= "(99.38,62.13)"
%	 fill-color= "#ffffff"
%	 p2= "(99.38,63.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(10.62,73.37)"
%	 fill-style= "solid"
%	 p1= "(9.38,72.13)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,73.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,73.37)"
%	 fill-style= "solid"
%	 p1= "(16.88,72.13)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,73.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(25.62,73.37)"
%	 fill-style= "solid"
%	 p1= "(24.38,72.13)"
%	 fill-color= "#ffffff"
%	 p2= "(24.38,73.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.12,73.37)"
%	 fill-style= "solid"
%	 p1= "(31.88,72.13)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,73.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.62,73.37)"
%	 fill-style= "solid"
%	 p1= "(39.38,72.13)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,73.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(48.12,73.37)"
%	 fill-style= "solid"
%	 p1= "(46.88,72.13)"
%	 fill-color= "#ffffff"
%	 p2= "(46.88,73.37)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(55.62,73.37)"
%	 fill-style= "solid"
%	 p1= "(54.38,72.13)"
%	 fill-color= "#ffffff"
%	 p2= "(54.38,73.37)"
%	 stroke-width= "0.15"
%	 />
%</g>
%<g>
%<circle closure= "plain"
%	 p3= "(10.62,88.12)"
%	 fill-style= "solid"
%	 p1= "(9.38,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,88.12)"
%	 fill-style= "solid"
%	 p1= "(16.88,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(25.62,88.12)"
%	 fill-style= "solid"
%	 p1= "(24.38,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(24.38,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.12,88.12)"
%	 fill-style= "solid"
%	 p1= "(31.88,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.62,88.12)"
%	 fill-style= "solid"
%	 p1= "(39.38,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(48.12,88.12)"
%	 fill-style= "solid"
%	 p1= "(46.88,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(46.88,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(55.63,88.12)"
%	 fill-style= "solid"
%	 p1= "(54.38,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(54.38,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(63.13,88.12)"
%	 fill-style= "solid"
%	 p1= "(61.88,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(61.88,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(70.62,88.12)"
%	 fill-style= "solid"
%	 p1= "(69.38,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(69.38,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(78.12,88.12)"
%	 fill-style= "solid"
%	 p1= "(76.88,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(76.88,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(85.62,88.12)"
%	 fill-style= "solid"
%	 p1= "(84.38,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(84.38,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(93.12,88.12)"
%	 fill-style= "solid"
%	 p1= "(91.88,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(91.88,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(100.62,88.12)"
%	 fill-style= "solid"
%	 p1= "(99.38,86.88)"
%	 fill-color= "#ffffff"
%	 p2= "(99.38,88.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(10.62,98.12)"
%	 fill-style= "solid"
%	 p1= "(9.38,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,98.12)"
%	 fill-style= "solid"
%	 p1= "(16.88,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(25.62,98.12)"
%	 fill-style= "solid"
%	 p1= "(24.38,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(24.38,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.12,98.12)"
%	 fill-style= "solid"
%	 p1= "(31.88,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.62,98.12)"
%	 fill-style= "solid"
%	 p1= "(39.38,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(48.12,98.12)"
%	 fill-style= "solid"
%	 p1= "(46.88,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(46.88,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(55.63,98.12)"
%	 fill-style= "solid"
%	 p1= "(54.38,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(54.38,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(70.62,98.12)"
%	 fill-style= "solid"
%	 p1= "(69.38,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(69.38,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(78.12,98.12)"
%	 fill-style= "solid"
%	 p1= "(76.88,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(76.88,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(85.62,98.12)"
%	 fill-style= "solid"
%	 p1= "(84.38,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(84.38,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(93.12,98.12)"
%	 fill-style= "solid"
%	 p1= "(91.88,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(91.88,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(100.62,98.12)"
%	 fill-style= "solid"
%	 p1= "(99.38,96.88)"
%	 fill-color= "#ffffff"
%	 p2= "(99.38,98.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(10.62,108.12)"
%	 fill-style= "solid"
%	 p1= "(9.38,106.88)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,108.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,108.12)"
%	 fill-style= "solid"
%	 p1= "(16.88,106.88)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,108.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.12,108.12)"
%	 fill-style= "solid"
%	 p1= "(31.88,106.88)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,108.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.62,108.12)"
%	 fill-style= "solid"
%	 p1= "(39.38,106.88)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,108.12)"
%	 stroke-width= "0.15"
%	 />
%</g>
%<g>
%<circle closure= "plain"
%	 p3= "(10.62,123.11)"
%	 fill-style= "solid"
%	 p1= "(9.38,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,123.11)"
%	 fill-style= "solid"
%	 p1= "(16.88,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(25.62,123.11)"
%	 fill-style= "solid"
%	 p1= "(24.38,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(24.38,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.11,123.11)"
%	 fill-style= "solid"
%	 p1= "(31.88,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.61,123.11)"
%	 fill-style= "solid"
%	 p1= "(39.38,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(48.11,123.11)"
%	 fill-style= "solid"
%	 p1= "(46.88,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(46.88,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(55.61,123.11)"
%	 fill-style= "solid"
%	 p1= "(54.38,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(54.38,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(63.11,123.11)"
%	 fill-style= "solid"
%	 p1= "(61.88,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(61.88,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(70.62,123.11)"
%	 fill-style= "solid"
%	 p1= "(69.38,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(69.38,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(78.12,123.11)"
%	 fill-style= "solid"
%	 p1= "(76.88,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(76.88,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(85.62,123.11)"
%	 fill-style= "solid"
%	 p1= "(84.38,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(84.38,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(93.12,123.11)"
%	 fill-style= "solid"
%	 p1= "(91.88,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(91.88,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(100.62,123.11)"
%	 fill-style= "solid"
%	 p1= "(99.38,121.87)"
%	 fill-color= "#ffffff"
%	 p2= "(99.38,123.11)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(10.62,133.12)"
%	 fill-style= "solid"
%	 p1= "(9.38,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(9.38,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(18.12,133.12)"
%	 fill-style= "solid"
%	 p1= "(16.88,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(16.88,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(25.62,133.12)"
%	 fill-style= "solid"
%	 p1= "(24.38,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(24.38,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(33.11,133.12)"
%	 fill-style= "solid"
%	 p1= "(31.88,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(31.88,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(40.61,133.12)"
%	 fill-style= "solid"
%	 p1= "(39.38,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(39.38,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(70.62,133.12)"
%	 fill-style= "solid"
%	 p1= "(69.38,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(69.38,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(78.12,133.12)"
%	 fill-style= "solid"
%	 p1= "(76.88,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(76.88,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(85.62,133.12)"
%	 fill-style= "solid"
%	 p1= "(84.38,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(84.38,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(93.12,133.12)"
%	 fill-style= "solid"
%	 p1= "(91.88,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(91.88,133.12)"
%	 stroke-width= "0.15"
%	 />
%<circle closure= "plain"
%	 p3= "(100.62,133.12)"
%	 fill-style= "solid"
%	 p1= "(99.38,131.88)"
%	 fill-color= "#ffffff"
%	 p2= "(99.38,133.12)"
%	 stroke-width= "0.15"
%	 />
%</g>
%<multicurve fill-style= "none"
%	 stroke-style= "dotted"
%	 stroke-width= "0.2"
%	 points= "(6.25,10);(6.25,10);(105,10);(105,10)"
%	 />
%<multicurve stroke-color= "#ffffff"
%	 fill-style= "none"
%	 points= "(0,136.25);(0,136.25);(0,128.75);(0,128.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,136.25)
\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](70,97.5)
(100,97.5)
(100,87.5)
(10,87.5)(70,97.5)
\pscustom[linestyle=none,fillcolor=gray,fillstyle=solid]{\psline(17.5,97.5)(10,97.5)
\psline(10,97.5)(17.5,107.5)
\psbezier(17.5,107.5)(17.5,107.5)(17.5,107.5)
\psline(17.5,107.5)(17.5,97.5)
\closepath}
\psline[linecolor=gray](10,107.5)(10,97.5)
\psline[linecolor=lightgray](10,72.5)(10,62.5)
\pscustom[linestyle=none,fillcolor=lightgray,fillstyle=solid]{\psline(10,62.5)(17.5,62.5)
\psline(17.5,62.5)(17.5,72.5)
\psbezier(17.5,72.5)(17.5,72.5)(17.5,72.5)
\psline(17.5,72.5)(10,62.5)
\closepath}
\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](10,97.5)(40,97.5)(40,87.5)(10,87.5)
\pspolygon[linestyle=none,fillcolor=gray,fillstyle=solid](55,87.5)
(10,87.5)
(47.5,97.5)
(55,97.5)(55,87.5)
\pspolygon[linestyle=none,fillcolor=gray,fillstyle=solid](40,97.5)
(10,97.5)
(32.5,107.5)
(40,107.5)(40,97.5)
\pspolygon[linestyle=none,fillcolor=gray,fillstyle=solid](10,132.5)(40,132.5)(40,122.5)(10,122.5)
\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](70,132.5)
(100,132.5)
(100,122.5)
(10,122.5)(70,132.5)
\rput(10,120){$1$}
\rput(17.5,120){$2$}
\rput(25,120){$3$}
\rput(32.5,120){$4$}
\rput(40,120){$5$}
\rput(47.5,120){$6$}
\rput(55,120){$7$}
\rput(62.5,120){$8$}
\rput(70,120){$9$}
\rput(77.5,120){$10$}
\rput(85,120){$11$}
\rput(92.5,120){$12$}
\rput(100,120){$13$}
\rput(10,135.62){$14$}
\rput(17.5,135.62){$15$}
\rput(25,135.62){$16$}
\rput(32.5,135.62){$17$}
\rput(40,135.62){$18$}
\rput(104.38,122.5){$A$}
\rput(3.75,132.5){$B_1$}
\rput(105,132.5){$B_0$}
\rput(70,135.62){$1$}
\rput(77.5,135.62){$2$}
\rput(85,135.62){$3$}
\rput(92.5,135.62){$4$}
\rput(100,135.62){$5$}
\rput(47.5,85){$6$}
\rput(55,85){$7$}
\rput(62.5,85){$8$}
\rput(10,95){$14$}
\rput(17.5,95){$15$}
\rput(25,95){$16$}
\rput(32.5,95){$17$}
\rput(40,95){$18$}
\rput(10,110.62){$6$}
\rput(17.5,110.62){$7$}
\rput(32.5,110.62){$14$}
\rput(40,110.62){$15$}
\rput(47.5,100){$19$}
\rput(55,100){$20$}
\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](10,62.5)(40,62.5)(40,52.5)(10,52.5)
\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](55,52.5)
(10,52.5)
(47.5,62.5)
(55,62.5)(55,52.5)
\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](40,62.5)
(10,62.5)
(32.5,72.5)
(40,72.5)(40,62.5)
\pspolygon[linewidth=0.1,linecolor=gray,linestyle=none,fillcolor=lightgray,fillstyle=solid](70,62.5)
(100,62.5)
(100,52.5)
(10,52.5)(70,62.5)
\rput(62.5,50){$8$}
\rput(25,60){$16$}
\rput(60,65.62){$21$}
\rput(47.5,75.62){$16$}
\rput(55,75.62){$19$}
\rput(25,75.62){$8$}
\rput(70,85){$9$}
\rput(77.5,85){$10$}
\rput(85,85){$11$}
\rput(92.5,85){$12$}
\rput(100,85){$13$}
\rput(70,50){$9$}
\rput(77.5,50){$10$}
\rput(85,50){$11$}
\rput(92.5,50){$12$}
\rput(100,50){$13$}
\psline{|*-|*}(100,20)(100,10)
\psline{|*-|*}(92.5,20)(92.5,10)
\psline{|*-|*}(85,20)(85,10)
\psline{|*-|*}(77.5,20)(77.5,10)
\psline{|*-|*}(70,20)(70,10)
\psline{|*-|*}(100,30.62)(100,20.62)
\psline{|*-|*}(92.5,30.62)(92.5,20.62)
\psline{|*-|*}(85,30.62)(85,20.62)
\psline{|*-|*}(77.5,30.62)(77.5,20.62)
\psline{|*-|*}(70,30.62)(70,20.62)
\psline{|*-|*}(40,10)(40,0)
\psline{|*-|*}(32.5,10)(32.5,0)
\psline{|*-|*}(25,10)(25,0)
\psline{|*-|*}(17.5,10)(17.5,0)
\psline{|*-|*}(10,10)(10,0)
\psline{|*-|*}(62.5,18.75)(62.5,8.75)
\psline{|*-|*}(47.5,15.62)(47.5,5.62)
\psline{|*-|*}(55,15.62)(55,5.62)
\psline{|*-|*}(62.5,29.38)(62.5,19.38)
\psline{|*-|*}(47.5,26.25)(47.5,16.25)
\psline{|*-|*}(55,27.5)(55,17.5)
\psline{|*-|*}(40,25)(40,15)
\psline{|*-|*}(32.5,25)(32.5,15)
\psline{|*-|*}(25,23.75)(25,13.75)
\psline{|*-|*}(17.5,22.5)(17.5,12.5)
\psline{|*-|*}(10,20.62)(10,10.62)
\rput(110,10){$A$}
\psline[linewidth=0.2,linestyle=dotted](6.25,20.62)(41.25,20.62)
\rput(110,21.25){$B$}
\psline{|*-|*}(47.5,36.88)(47.5,26.88)
\psline{|*-|*}(55,38.12)(55,28.12)
\psline{|*-|*}(32.5,35.62)(32.5,25.62)
\psline{|*-|*}(40,35.62)(40,25.62)
\psline{|*-|*}(25,34.38)(25,24.38)
\psline{|*-|*}(17.5,33.12)(17.5,23.12)
\psline{|*-|*}(10,31.25)(10,21.25)
\psline[linewidth=0.2,linestyle=dotted](6.25,31.25)(105,31.25)
\rput(110,31.88){$C$}
\psline[linewidth=0.2,linestyle=dotted](45.62,20.62)(56.25,20.62)
\psline[linewidth=0.2,linestyle=dotted](70,20.62)(105,20.62)
\rput(28.75,22.5){$B_1$}
\rput(51.25,22.5){$B_2$}
\rput(81.25,22.5){$B_0$}
\psline[linewidth=0.2,linestyle=dotted](60,20.62)(65.62,20.62)
\rput(65.62,22.5){$B_3$}
\rput(59.38,98.75){$B_2$}
\rput(65.62,65.62){$B_3$}
\rput(32.5,60){$17$}
\rput(40,60){$18$}
\newrgbcolor{userFillColour}{0.58 0.58 0.58}
\pscustom[linestyle=none,fillcolor=userFillColour,fillstyle=solid]{\psline(25,62.5)(10,62.5)
\psline(10,62.5)(25,72.5)
\psbezier(25,72.5)(25,72.5)(25,72.5)
\psline(25,72.5)(25,62.5)
\closepath}
\newrgbcolor{userFillColour}{0.58 0.58 0.58}
\pscustom[linestyle=none,fillcolor=userFillColour,fillstyle=solid]{\psline(47.5,62.5)(10,62.5)
\psline(10,62.5)(47.5,72.5)
\psbezier(47.5,72.5)(47.5,72.5)(47.5,72.5)
\psline(47.5,72.5)(47.5,62.5)
\closepath}
\pscustom[linestyle=none,fillcolor=gray,fillstyle=solid]{\psline(55,62.5)(10,62.5)
\psline(10,62.5)(55,72.5)
\psbezier(55,72.5)(55,72.5)(55,72.5)
\psline(55,72.5)(55,62.5)
\closepath}
\pscustom[linestyle=none,fillcolor=gray,fillstyle=solid]{\psline(62.5,52.5)(10,52.5)
\psline(10,52.5)(62.5,62.5)
\psbezier(62.5,62.5)(62.5,62.5)(62.5,62.5)
\psline(62.5,62.5)(62.5,52.5)
\closepath}
\rput(55,60){$20$}
\rput(47.5,60){$19$}
\rput{0}(10,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(25,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.5,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(40,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(47.5,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(62.5,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(70,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(77.5,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(85,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(92.5,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100,52.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(25,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.5,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(40,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(47.5,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(62.5,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(70,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(77.5,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(85,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(92.5,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100,62.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10,72.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,72.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(25,72.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.5,72.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(40,72.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(47.5,72.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55,72.75){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(25,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.5,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(40,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(47.5,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.01,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(62.51,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(70,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(77.5,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(85,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(92.5,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100,87.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(25,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.5,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(40,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(47.5,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(55.01,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(70,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(77.5,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(85,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(92.5,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100,97.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10,107.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,107.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.5,107.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(40,107.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(25,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.49,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\rput{0}(40,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\rput{0}(47.5,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\rput{0}(55,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\rput{90}(62.5,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\rput{0}(70,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(77.5,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(85,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(92.5,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100,122.49){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(10,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(17.5,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(25,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(32.5,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\rput{0}(40,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.87,0.87)}
\rput{0}(70,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(77.5,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(85,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(92.5,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\rput{0}(100,132.5){\psellipse[linewidth=0.15,fillcolor=white,fillstyle=solid](0,0)(0.88,0.88)}
\psline[linewidth=0.2,linestyle=dotted](6.25,10)(105,10)
\psline[linecolor=white](0,136.25)(0,128.75)
\end{pspicture}

